Efficient Prior-Free Mechanisms for No-Regret Agents

We study a repeated Principal Agent problem between a long lived Principal and Agent pair in a prior free setting. In our setting, the sequence of realized states of nature may be adversarially chosen, the Agent is non-myopic, and the Principal aims for a strong form of policy regret. Following Camara, Hartline, and Johnson, we model the Agent's long-run behavior with behavioral assumptions that relax the common prior assumption (for example, that the Agent has no swap regret). Within this framework, we revisit the mechanism proposed by Camara et al., which informally uses calibrated forecasts of the unknown states of nature in place of a common prior. We give two main improvements. First, we give a mechanism that has an exponentially improved dependence (in terms of both running time and regret bounds) on the number of distinct states of nature. To do this, we show that our mechanism does not require truly calibrated forecasts, but rather forecasts that are unbiased subject to only a polynomially sized collection of events -- which can be produced with polynomial overhead. Second, in several important special cases -- including the focal linear contracting setting -- we show how to remove strong ``Alignment'' assumptions (which informally require that near-ties are always broken in favor of the Principal) by specifically deploying ``stable'' policies that do not have any near ties that are payoff relevant to the Principal. Taken together, our new mechanism makes the compelling framework proposed by Camara et al. much more powerful, now able to be realized over polynomially sized state spaces, and while requiring only mild assumptions on Agent behavior.

==> some_backup.tex <==
\section{Alternative assumptions -- toy result for two actions}
Consider a game with only two actions, i.e., $\abs{\cR} =2$.
\begin{assumption}[no secret info.]\label{asp:no-xswap-reg-subsequence}Assume that for any $p,r,y$, on the subsequence with $(p_t,\rho_t,y_t) = (p,r,y)$, the agent does not perform much better than the principal's recommendation, i.e.,
    \begin{align*}
        \frac{1}{n_{p,r,y}}\sum_{t=1}^T\ind{(p_t,\rho_t,y_t) = (p,r,y)} \left(U(r_t, p_t,y_t)- U(r, p_t,y_t)\right)\leq \frac{1}{\sqrt{{n_{p,r,y}}}}\,,
    \end{align*}
    where $n_{p,r,y} = \sum_{t=1}^T\ind{(p_t,\rho_t,y_t) = (p,r,y)}$.
\end{assumption}
\begin{assumption}[no tie-breaking for every state.]\label{asp:tie-breaking}
    For any policy $p$ and state $y\in \cY$, we have 
    \begin{align*}
        U(r_1,p,y)\neq U(r_2,p,y)\,.
    \end{align*}
    Let $\delta :=\min_{y\in \cY} \abs{U(r_1,p,y)-U(r_2,p,y)}$. Then we have $\delta>0$.
\end{assumption}

\begin{lemma}[small disagreement region]
    For any sequence of $p_t,\rho_t$,
    under the assumptions of no internal regret (Assumption~\ref{asp-alt:no-internal-reg}), no secret information (Assumption~\ref{asp:no-xswap-reg-subsequence}) and no tie-breaking for every state (Assumption~\ref{asp:tie-breaking}), we have 
    \begin{align*}
        \sum_{t=1}^T\ind{\rho_t\neq r_t}\leq \frac{\ir + (1+\delta)\sum_{p,r_1,y}\frac{\sqrt{{n_{p,r_1,y}}}}{\delta}}{\delta}\,,
    \end{align*}
    where $\ir =\max_{h}\frac{1}{T}\sum_{t=1}^T (U(h(p_t,\rho_t,r_t),p_t, y_t) - U(r_t,p_t,y_t))$.
\end{lemma}
\begin{proof}
    Consider the subsequence $\{t|(p_t,\rho_t) = (p,r_1)\}$, our goal is to upper bound the number of rounds $r_t = r_2\neq r_1$ in this subsequence.
    Let $n_{p,r_1,y, r_2} = \sum_{t=1}^T\ind{(p_t,\rho_t,y_t,r_t) = (p,r_1,y,r_2)}$. 
    By Assumption~\ref{asp:no-xswap-reg-subsequence}, we have that for all $y\in \cY$,
    \begin{align*}
        &\sum_{t=1}^T\ind{(p_t,\rho_t,y_t,r_t) = (p,r_1,y,r_2)}\left(U(r_2, p,y)- U(r_1, p,y)\right)\\
        =&\sum_{t=1}^T\ind{(p_t,\rho_t,y_t) = (p,r_1,y)}\left(U(r_t, p_t,y_t)- U(r, p_t,y_t)\right)
        \leq \sqrt{{n_{p,r_1,y}}}\,.
    \end{align*}
    For $y$ satisfying $U(r_2, p,y)> U(r_1, p,y)$, we have
    \begin{align*}
        n_{p,r_1,y, r_2}\leq \frac{\sqrt{{n_{p,r,y}}}}{\left(U(r_2, p,y)- U(r_1, p,y)\right)} \leq \frac{\sqrt{{n_{p,r,y}}}}{\delta} \,.
    \end{align*}
    On the other hand, we have
    \begin{align*}
         &\sum_{y\in \cY}n_{p,r_1,y, r_2}\left(U(r_1,p,y) - U(r_2,p,y)\right)\\
        =&\sum_{t=1}^T\ind{(p_t,\rho_t,r_t) = (p,r_1,r_2)}\left(U(r_1,p,y_t) - U(r_2,p,y_t)\right)\leq \ir_{p,r_1}\,,
    \end{align*}
    which is small by Assumption~\ref{asp-alt:no-internal-reg}.
    By re-arranging terms, we have
    \begin{align*}
        &\sum_{y\in \cY}n_{p,r_1,y, r_2}\ind{U(r_2,p,y) < U(r_1,p,y)}\left(U(r_1,p,y) - U(r_2,p,y)\right)\\
        \leq& \ir_{p,r_1} + \sum_{y\in \cY}n_{p,r_1,y, r_2}\ind{U(r_2,p,y) > U(r_1,p,y)}\left(U(r_2,p,y) - U(r_1,p,y)\right)\\
        \leq& \ir_{p,r_1} + \sum_{y\in \cY}\frac{\sqrt{{n_{p,r_1,y}}}}{\delta}\ind{U(r_2,p,y) > U(r_1,p,y)}\\
        \leq&  \ir_{p,r_1} + \sum_{y\in \cY}\frac{\sqrt{{n_{p,r_1,y}}}}{\delta}\,.
    \end{align*}
    Therefore, we have
    \begin{align*}
        \sum_{y\in \cY}n_{p,r_1,y, r_2}\ind{U(r_2,p,y) < U(r_1,p,y)}\leq \frac{\ir_{p,r_1} + \sum_{y\in \cY}\frac{\sqrt{{n_{p,r_1,y}}}}{\delta}}{\delta}\,.
    \end{align*}
    Then we have
    \begin{align*}
        \sum_{t=1}^T\ind{(p_t,\rho_t,r_t) = (p,r_1,r_2)}= \sum_{y\in \cY}n_{p,r_1,y, r_2}\leq \frac{\ir_{p,r_1} + (1+\delta)\sum_{y\in \cY}\frac{\sqrt{{n_{p,r_1,y}}}}{\delta}}{\delta}\,.
    \end{align*}
    By summing over all $(p,r)$, we have
    \begin{align*}
         \sum_{t=1}^T\ind{\rho_t\neq r_t}= \sum_{(p,r_1)}\sum_{t=1}^T\ind{(p_t,\rho_t,r_t) = (p,r_1,r_2)}\leq \frac{\ir + (1+\delta)\sum_{p,r_1,y}\frac{\sqrt{{n_{p,r_1,y}}}}{\delta}}{\delta}\,.
    \end{align*}
\end{proof}


==> src/camara.tex <==
\section{Comparison to \cite{camara2020mechanisms}\hsedit{tbd}}
\subsection{A set of alternative assumptions}
In this section, we propose a set of alternative assumptions, which are weaker than assumptions in \cite{camara2020mechanisms}.
The main difference of assumptions in this subsection from those in Section~\ref{sec:general} is that under the constant mechanism $\sigma^{p_0}$, the signal $I_t$ in round $t$ is $(p_t,r_t,p^0,r^{p_0}_t, a^{p_0}_t)$ instead of $(p^0,r^{p_0}_t, a^{p_0}_t)$.

\begin{definition}[finer multi-calibration error of the forecast]
We consider the calibration error on finer partition of the sequence.
For the proposed mechanism $\sigma^\dagger$, similar to Definition~\ref{def:principal-cal}, we consider the calibration error on the subsequences defined by the policy and the recommendation.
For the fixed constant mechanisms $\{\sigma^{p_0}\}_{p_0\in \cP}$, we consider the calibration error on the subsequences defined by the policy, the recommendation and the policy-recommmendation under the proposed mechanism.
forand the calibration error on the subsequences defined by the policy, the recommendation for
Specifically, let $E' = \{S_{p,r}|(p,r)\in \cP\times \cA\} \cup \{S''_{p_0,r,p',r'}|(p_0,r,p',r')\in \cP\times \cA\times \cP\times \cA\}$ where
\begin{equation*}
    S_{p,r} = \{\pi| \brp(\pi) = p , \brr(p,\pi) =r\}\,,
\end{equation*}
and 
\begin{equation*}
    S''_{p_0,r,p',r'} : = \{\pi|\brr(p_0,\pi) =r, \brp(\pi) = p' , \brr(p',\pi) =r'\}\,.
\end{equation*}
We say the multi-calibration error is upper bounded by $\alpha'$ if $\calerr(S)\leq \alpha'$ for all $S\in E'$.
\end{definition}

\begin{definition}[signal]
    Under the proposed mechanism $\sigma^\dagger$, the signal $I^\dagger_t = (p_t,r_t,a_t)$ is the triple of the policy, the recommendation and the action.
    Under the constant mechanism $p_0\in \cP$, the signal $I^{p_0}_t = (p_t,r_t,p^0,r^{p_0}_t, a^{p_0}_t)$ is a tuple of the policy and the recommendation under $\sigma^\dagger$, and the policy, the recommendation and the action under $\sigma^{p_0}$. 
\end{definition}

\begin{assumptionp}{\ref*{asp:alignment}$'$}[alignment]\label{asp-alt:alignment}
   We assume that there exists a constant $M>0$ such that for any prior distribution $\pi$ and signal structure $\gamma$, for any $\epsilon$-approximately optimal response $\mu^\epsilon(\gamma, p^*(\pi),\pi)$ to $(\gamma, p^*(\pi),\pi)$, we have
    \begin{align}
        &V(a^*(p^*(\pi), \pi), p^*(\pi), \pi)-\EEs{y\sim \pi}{\EEs{I\sim \gamma(\cdot, y)}{V(\mu_I^\epsilon(\gamma, p^*(\pi),\pi), p^*(\pi),y)}}\nonumber\\
        \leq& M (\EEs{y\sim \pi}{\EEs{I\sim \gamma(\cdot, y)}{U(a^*_I(\gamma, p^*(\pi),\pi), p^*(\pi),y)}} - U(a^*(p^*(\pi), p^*(\pi), \pi) ) + \epsilon\,;\label{eq:alignment-alt}
    \end{align}
   and for any fixed policy $p_0\in \cP$, for any $\epsilon$-approximately optimal response $\mu^\epsilon(\gamma, p_0,\pi)$ to $(\gamma, p_0,\pi)$, we have
    \begin{align}
        &\EEs{y\sim \pi}{\EEs{I\sim \gamma(\cdot, y)}{V(\mu_I^\epsilon(\gamma, p_0,\pi), p_0,y)}}-\max_{p'\in \cP}V(a^*(p',\pi),p', \pi)\nonumber\\
        \leq& M (\EEs{y\sim \pi}{\EEs{I\sim \gamma(\cdot, y)}{U(a_I^*(\gamma, p_0,\pi), p_0,y)}} -  U(a^*(p_0), p_0, \pi) ) +  \epsilon\,.\label{eq:alignment-alt-2}
    \end{align}
\end{assumptionp}

\begin{assumptionp}{\ref*{asp:no-internal-reg}$'$}[no finer counterfactual internal regret for Agent]\label{asp-alt:no-finer-internal-reg}
Let $\ecf$ be an upper bound on the counterfactual internal regret with the context being the signal for the realized sequence of states $y_{1:T}$ and realized sequence of policies and recommendations generated by either the proposed mechanism or the constant mechanisms.
That is,
    \begin{equation*}        \cir(y_{1:T},p_{1:T},r_{1:T}):=\max_{h:\cP \times \cA\times \cA\mapsto \cA}\frac{1}{T}\sum_{t=1}^T (U(h(p_t,r_t,a_t),p_t, y_t) - U(a_t,p_t,y_t)) \leq \ecf\,,
    \end{equation*}
    and for all $p_0\in \cP$,
    \begin{equation*}        
    \cir(y_{1:T},(p_0,\ldots,p_0),r^{p_0}_{1:T}):=\max_{h:\cP^2\times \cA^3\mapsto \cA}\frac{1}{T}\sum_{t=1}^T (U(h(p_t,r_t, p_0, r^{p_0}_t,a^{p_0}_t),p_0, y_t) - U(a^{p_0}_t,p_0,y_t)) \leq \ecf\,.
    \end{equation*}
    We assume that there exists a small $\ecf$.
% Let $\eint$ be an upper bound on the internal regret with context of $(p_t,\rho_t, p^*_t, \rho^*_t, r_t)$ for the realized sequence of states $y_{1:T}$ and realized sequence of policies $p_{1:T}$ and recommendations $\rho_{1:T}$ generated by either the proposed mechanism or the constant mechanisms.
\end{assumptionp}

% \begin{assumption}[Agent has no secret information.]\label{asp:no-sec-info}
% Let $\eneg$ be an upper bound on the negative cross-swap regret for the realized sequence of states $y_{1:T}$ and realized sequence of policies $p_{1:T}$ and recommendations $\rho_{1:T}$ generated by the proposed mechanism and constant mechanisms.
% That is,
%     \begin{equation*}
%         \nr(y_{1:T},p^*_{1:T},\rho^{*}_{1:T}):=\frac{1}{T}\sum_{t=1}^T U(r^*_t,p^*_t,y_t)- \max_{h:\cP\times \cA\mapsto \cA} \frac{1}{T}\sum_{t=1}^T U(h(p^*_t, \rho^{*}_t),p^*_t,y_t) \leq\eneg\,,
%     \end{equation*}
%     and for all $p\in \cP$,
%     \begin{equation*}
%         \nr(y_{1:T},(p,\ldots,p),\rho^{p}_{1:T}):=\frac{1}{T}\sum_{t=1}^T U(r^p_t,p,y_t)- \max_{h:\cP\times \cA\mapsto \cA} \frac{1}{T}\sum_{t=1}^T U(h(p, \rho^{p}_t),p,y_t) \leq\eneg\,.
%     \end{equation*}
%     We assume that there exists a small $\eneg$.
% \end{assumption}


\begin{theorem}
    Under Assumptions~\ref{asp-alt:alignment}, \ref{asp-alt:no-finer-internal-reg},\ref{asp:no-sec-info}, the Principal's regret satisfies that 
    \begin{equation*}
        \textrm{PR}(L, y_{1:T}) \leq \cO(\abs{\cP}\abs{\cA}\alpha + \eint + \eneg).
    \end{equation*}
\end{theorem}
\begin{proof}
    To prove the theorem, we will prove that
\begin{equation*}
     \frac{1}{T}\sum_{t=1}^T V(r_t^*,p_t,y_t)\geq \frac{1}{T}\sum_{t=1}^T V(\rho^{*}_t,p_t,y_t)-(M+1)T\eint-MT\eneg -(4M+2)\calerr(\pip)\,,
\end{equation*}
and for all $p\in \cP$
\begin{equation*}
     \frac{1}{T}\sum_{t=1}^T V(r_t^p,p,y_t)\leq \frac{1}{T}\sum_{t=1}^T V(\rho^{*}_t,p_t,y_t) +  (M+1)T\eint + MT \eneg\,.
\end{equation*}
The first part has been proved in Lemma~\ref{lmm:utility-difference}. We only need to prove the second part.
For any constant mechanism $\sigma^p$, now we consider the subsequence in which $\brp(\pip_t) = p' , \brr(p',\pip_t) =\rho',\brr(p,\pip_t) =\rho$. 
Let $t\in (p,\rho,p',\rho')$ to present $t: \brp(\pip_t) = p' , \brr(p',\pip_t) =\rho',\brr(p,\pip_t) =\rho$.
In this subsequence, we let the signal structure be $\hat\gamma_{p,\rho,p',\rho'}((p,\rho,r), y) := \frac{\sum_{t\in (p,\rho,p',\rho')} \ind{r^p_t = r, y_t = y}}{\sum_{t\in (p,\rho,p',\rho')} \ind{y_t = y}}$.
Then we have
\begin{align*}
        &\EEs{y\sim \pip_{p,\rho,p',\rho'}}{\EEs{J\sim \hat \gamma_{p,\rho,p',\rho'}(\cdot,y)}{U(r_J,p,y)}} \\
        \geq & \max_{r_I} \EEs{y\sim \pip_{p,\rho,p',\rho'}}{\EEs{J\sim \hat \gamma_{p,\rho,p',\rho'}(\cdot,y)}{U(r_J,p,y)}}- \frac{1}{n_{p,\rho,p',\rho'}}\ir^p_{p,\rho,p',\rho'} -2\norm{\pip_{p,\rho,p',\rho'}  - \hat y_{p,\rho,p',\rho'}}_1 \,. 
    \end{align*}
    and
\begin{align*}
    &\max_{r_I} \EEs{y\sim \pip_{p,\rho,p',\rho'}}{\EEs{J\sim \hat \gamma_{p,\rho,p',\rho'}(\cdot,y)}{U(r_J,p,y)}}-\max_{\tilde r}\EEs{y\sim \pip_{p,\rho,p',\rho'}}{U(\tilde r,p,y)}\\
    \leq&  \frac{1}{n_{p,\rho,p',\rho'}}\nr^p_{p,\rho,p',\rho'}+\frac{1}{n_{p,\rho,p',\rho'}}\ir^p_{p,\rho,p',\rho'} +4\norm{\pip_{p,\rho,p',\rho'}  -\hat y_{p,\rho,p',\rho'}}_1\,.
\end{align*}
Then combining with Assumption~\ref{asp-alt-ver2:alignment}, we have
\begin{align}
    &\EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}\nonumber\\
    \leq& \EEs{y\sim \pip_{p,r}}{V(\tilde r(p),p,y)} + M(\frac{1}{n_{p,r}}\nr^p_{p,r}+\frac{1}{n_{p,r}}\ir^p_{p,r} +4\norm{\pip_{p,r}  -\hat y_{p,r}}_1) \nonumber\\
    &+ \frac{1}{n_{p,r}}\ir^p_{p,r} +2\norm{\pip_{p,r}  - \hat y_{p,r}}_1    
    \,.\label{eq:step3}
\end{align}
For the first term, we have
\begin{align*}
    &\EEs{y\sim \pip_{p,r}}{V(\tilde r( p),p,y)}=\EEs{y\sim \pip_{p,r}}{V(\brr(\tilde p, \pip_{p,r}), p,y)} \tag{defn of $\tilde r$}\\
    =& \frac{1}{n_{p,r}}\sum_{t\in (p,r)} V(\brr( p, \pip_{p,r}), p,\pip_t)= \frac{1}{n_{p,r}}\sum_{t\in (p,r)} V(r, p,\pip_t)
\end{align*}
Therefore, we have
\begin{align*}
    &\sum_{t=1}^TV(r^p_t,p,y_t) =\sum_{r}\sum_{t\in (p,r)}V(r^p_t,p,y_t)\\
    =& \sum_{r}n_r \EEs{y\sim \hat y_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}\\
    \leq & \sum_{r}n_r \EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}+ \calerr(\pip,p,r)\\
    \leq & \sum_{r}n_r \left(\EEs{y\sim \pip_{p,r}}{V(\tilde r(p),p,y)} + \frac{1}{n_{p,r}}M\nr^p_{p,r}+\frac{1}{n_{p,r}}(M+1)\ir^p_{p,r} +(4M+2)\norm{\pip_{p,r}  -\hat y_{p,r}}_1\right)\\
    &+ \calerr(\pip,p,r)\tag{Eq~\eqref{eq:step3}}\\
    = & \sum_{r}n_r \left(\EEs{y\sim \pip_{p,r}}{V(r,p,y)} + \frac{1}{n_{p,r}}M\nr^p_{p,r}+\frac{1}{n_{p,r}}(M+1)\ir^p_{p,r} +(4M+2)\norm{\pip_{p,r}  -\hat y_{p,r}}_1\right)\\
    &+ \calerr(\pip,p,r)\\
    % = &\sum_{r}n_r \left(\max_{\tilde p}\EEs{y\sim \hat y_{p,r}}{V(\tilde r(\tilde p),\tilde p,y)}+ M(\ir^p_{p,r} + \nr^p_{p,r}) + \ir^p_{p,r}\right)\\
    \leq &\sum_{t=1}^T V(\rho^{\tilde p}_t, p,y_t)  +  (M+1)T\eint + MT \eneg+(4M+4)\calerr(\pip)\,.
\end{align*}
\end{proof}

\subsection{Comparison to Theorem~5 of \cite{camara2020mechanisms}}
\cite{camara2020mechanisms} adopt $\epsilon$-robust policy.
The $\epsilon$-robust policy is worst-case optimal over all $\epsilon$-approximately optimal response distributions.
Formally, for any $p,\pi,\epsilon$, let $\cB(\pi,p,\epsilon)$ denote the set of all $\epsilon$-approximately optimal response distributions, i.e., 
\begin{equation*}
        \cB(\pi,p,\epsilon)=\{\mu\in \Delta(\cR)|\max_{\tilde r}\EEs{y\sim \pi}{U(\tilde r,p,y)} - \EEs{y\sim \pi}{\EEs{r\sim \mu}{U(r,p,y)}}\leq \epsilon\}\,.
\end{equation*}
The $\epsilon$-robust policy is $\argmax_{p\in \cP} \min_{r\in \cB(\pi,p,\epsilon)}$. Similarly, when there is a signal structure $\gamma$, let $\cB(\pi,p,\gamma,\epsilon)$ denote denotes the set of all $\epsilon$-approximately optimal responses given the signal $I$, i.e.,
    \begin{equation*}
        \cB(\pi,p,\gamma,\epsilon)=\left\{\mu_I\in\Delta(\mathcal{R})\mid\max_{\tilde{r}_I\in\mathcal{R}}\EEs{y\sim\pi}{\EEs{J
        \sim\gamma(\cdot,y)}{U(\tilde{r}_J,p,y)-\EEs{r\sim\mu_I}{U(r,p,y)}}}\leq \epsilon\right\}\,.
    \end{equation*}
    
\begin{assumption}[bounded cost of $\epsilon$-robustness]\label{camara-asp:eps-robust}
    For any distribution $\pi$, 
    \begin{equation*}
        \max_{p\in \cP} \max_{r\in \cB(\pi,p,\epsilon)}U(r,p,\pi) - \max_{p\in \cP} \min_{r\in \cB(\pi,p,\epsilon)}U(r,p,\pi) = \cO(\epsilon)\,.
    \end{equation*}
\end{assumption}
\begin{assumption}[$\epsilon$-bounded FCIR]\label{camara-asp:fcir}
\begin{equation*}
    \max_{h}\frac{1}{T}\sum_{t=1}^T (U(h(\pip_t,r_t^*,(r_t^p)_{p\in\cP}),p_t, y_t) - U(r_t,p_t,y_t)) \leq \epsilon\,.
\end{equation*}    
\end{assumption}
\begin{assumption}[$\tilde \epsilon$-lower bounded FER]\label{camara-asp:fer}
    \begin{equation*}
    \max_{h}\frac{1}{T}\sum_{t=1}^T (U(h(\pip_t),p_t, y_t) - U(r_t,p_t,y_t)) \geq -\tilde \epsilon\,.
\end{equation*} 
\end{assumption}
\begin{assumption}[Alignment. Assumption 9 of \cite{camara2020mechanisms}]\label{camara-asp:alignment}
For any prior distribution $\pi$, let $p^*(\pi)$ denote the policy deployed by the Principal when the forecast is $\pi$.
There exists a constant $M_1>0$ and a small $\epsilon>0$ s.t. for any prior distribution $\pi$ and signal structure $\gamma$,
    \begin{align*}
        &\min_{r\in \cB(\pi,p^*(\pi),\bar \epsilon)} V(r,p^*(\pi),\pi) - \min_{r_I\in \cB(\pi,p^*(\pi),\gamma,\bar \epsilon)}\EEs{y\sim \pi, I\sim \gamma(\cdot,y)}{V(r_I,p^*(\pi),y)}\\
        \leq& M_1\left( \max_{(r_I)_{I\in \cI}}\EEs{y\sim \pi,I\sim \gamma(\cdot,y)}{U(r_I,p^*(\pi),y)}-\max_r U(r,p^*(\pi),\pi) \right) +\epsilon\,,
    \end{align*}
    and 
    \begin{align*}
        &\max_{r_I\in \cB(\pi,p,\gamma,\bar \epsilon)}\EEs{y\sim \pi, I\sim \gamma(\cdot,y)}{V(r_I,p,y)}-\max_{\tilde p\in \cP}\max_{r\in \cB(\pi,\tilde p,\bar \epsilon)} V(r,p,\pi) \\
        \leq& M_1\left( \max_{(r_I)_{I\in \cI}}\EEs{y\sim \pi,I\sim \gamma(\cdot,y)}{U(r_I,p,y)}-\max_r U(r,p,\pi) \right) +\epsilon\,.
    \end{align*}

\end{assumption}
\begin{remark}
    Note that the deployed policy in \cite{camara2020mechanisms} is the $\epsilon$-robust policy $p^*(\pi) = \argmax_{p\in \cP} \min_{r\in \cB(\pi,p,\epsilon)}$ instead of $\brp(\pi)$ as we did in this work. Besides, the signal in our work is the action $I_t = r_t$ taken by the Agent while in \cite{camara2020mechanisms}, the signal is $I'_t = (\pip_t, r_t^*, (r^p_t)_{p\in \cP})$.
    Since no matter what mechanism is implemented, $I_t$ is always contained in $I'_t$, hence, for any structure $\gamma$ in our setting, we could define a corresponding structure $\gamma'$ with invariant $\pip_t$ and $r_t = r^*_t = r^p_t$ for all $p\in \cP$.
\end{remark}
\begin{theorem}[Theorem 5 of \cite{camara2020mechanisms}]
    Under Assumptions~\ref{camara-asp:eps-robust}, \ref{camara-asp:fcir}, \ref{camara-asp:fer} and \ref{camara-asp:alignment}, given that the forecast is fully calibrated, the Principal's regret is bounded.
\end{theorem}
We compare the assumptions in Table~\ref{tab:asp-compare}. 
\begin{table}[H]
    \centering
    \begin{tabular}{c|c}
    ours & \citep{camara2020mechanisms}  \\\hline
     Principal forecast calibration (Assumption~\ref{asp:principal-cal}) & full calibration \\\hline
     Agent's forecast calibration (Assumption~\ref{asp:agent-cal})& \multirow{2}{*}{bounded FCIR (Assumption~\ref{camara-asp:fcir})} \\
     bounded internal regret (Assumption~\ref{asp-alt:no-internal-reg})&\\\hline
     lower bounded cross-swap regret (Assumption~\ref{asp:no-sec-info})& lower bounded FER (Assumption~\ref{camara-asp:fer})\\\hline
     Agent's utility margin (Assumption \ref{asp:utility-margin})& \multirow{2}{*}{alignment (Assumption~\ref{camara-asp:alignment})}\\
     alignment (Assumption~\ref{asp-alt:alignment})&\\\hline
     & bounded cost of $\epsilon$-robustness (Assumption~\ref{camara-asp:eps-robust})\\\hline
    \end{tabular}
    \caption{Comparison of assumptions}
    \label{tab:asp-compare}
\end{table}

\begin{lemma}
For any prior distribution $\pi$, let $p^*(\pi)$ denote the deployed policy. Under Assumption~\ref{camara-asp:eps-robust}, if Assumption~\ref{camara-asp:alignment} $\Rightarrow$ holds for $p^*(\cdot)$ and signal structure $\gamma$, then  Assumption~\ref{asp-alt:alignment} holds.\todohs{not right and not finished} 
\end{lemma}
\begin{proof}
By Assumption~\ref{camara-asp:alignment}, we have
    \begin{align*}
        &\min_{r\in \cB(\pi,p^*(\pi),\bar \epsilon)} V(r,p^*(\pi),\pi) - \min_{r_I\in \cB(\pi,p^*(\pi),\gamma,\bar \epsilon)}\EEs{y\sim \pi, I\sim \gamma(\cdot,y)}{V(r_I,p^*(\pi),y)}\\
        \leq& M_1\left( \max_{(r_I)_{I\in \cI}}\EEs{y\sim \pi,I\sim \gamma(\cdot,y)}{U(r_I,p^*(\pi),y)}-\max_r U(r,p^*(\pi),\pi) \right)+\epsilon\,.
    \end{align*}
    Since
    \begin{align*}
        \min_{r\in \cB(\pi,p^*(\pi),\bar \epsilon)} V(r,p^*(\pi),\pi) \geq& V(\tilde r(p^*(\pi)),p^*(\pi),\pi) - \bar \epsilon\tag{Assumption~\ref{camara-asp:eps-robust}}
    \end{align*}
    and for any $\bar \epsilon$-approximately optimal respond $(r_I^{\bar \epsilon})_{I\in \cI}$,
    \begin{align*}
        \min_{r_I\in \cB(\pi,p^*(\pi),\gamma,\bar \epsilon)}\EEs{y\sim \pi, I\sim \gamma(\cdot,y)}{V(r_I,p^*(\pi),y)} \leq \EEs{y\sim \pi, I\sim \gamma(\cdot,y)}{V(r_I^{\bar \epsilon},p^*(\pi),y)}\,,
    \end{align*}
    we have that 
    \begin{align*}
        &V(\tilde r(p^*(\pi)),p^*(\pi),\pi) - \bar \epsilon-\EEs{y\sim \pi, I\sim \gamma(\cdot,y)}{V(r_I^{\bar \epsilon},p^*(\pi),y)}\\
        \leq& M_1\left( \max_{(r_I)_{I\in \cI}}\EEs{y\sim \pi,I\sim \gamma(\cdot,y)}{U(r_I,p^*(\pi),y)}-\max_r U(r,p^*(\pi),\pi) \right)+\epsilon\,.
    \end{align*}
    By rearranging terms, we have
\begin{align*}
    &V(\tilde r(p^*(\pi)),p^*(\pi),\pi) - \EEs{y\sim \pi, I\sim \gamma(\cdot,y)}{V(r_I^{\bar \epsilon},p^*(\pi),y)}\\
        \leq& M_1\left( \max_{(r_I)_{I\in \cI}}\EEs{y\sim \pi,I\sim \gamma(\cdot,y)}{U(r_I,p^*(\pi),y)}-\max_r U(r,p^*(\pi),\pi) \right)+\epsilon+\bar \epsilon\,.
\end{align*}
Thus, we have proved the first part of Assumption~\ref{asp-alt:alignment}.
    The proof of the second part is similar.
    By Assumption~\ref{camara-asp:alignment}, we have 
    \begin{align*}
        &\max_{r_I\in \cB(\pi,p,\gamma,\bar \epsilon)}\EEs{y\sim \pi, I\sim \gamma(\cdot,y)}{V(r_I,p,y)}-\max_{\tilde p\in \cP}\max_{r\in \cB(\pi,\tilde p,\bar \epsilon)} V(r,p,\pi) \\
        \leq& M_1\left( \max_{(r_I)_{I\in \cI}}\EEs{y\sim \pi,I\sim \gamma(\cdot,y)}{U(r_I,p,y)}-\max_r U(r,p,\pi) \right)+\epsilon\,.
    \end{align*}
    For any $\bar \epsilon$-approximately optimal respond $(r_I^{\bar \epsilon})_{I\in \cI}$, we have
    \begin{align*}
        \max_{r_I\in \cB(\pi,p,\gamma,\bar \epsilon)}\EEs{y\sim \pi, I\sim \gamma(\cdot,y)}{V(r_I,p,y)}\geq \EEs{y\sim \pi, I\sim \gamma(\cdot,y)}{V(r_I^{\bar \epsilon},p,y)}\,.
    \end{align*}
    We also have
    \begin{align*}
        \max_{\tilde p\in \cP}\max_{r\in \cB(\pi,\tilde p,\bar \epsilon)} V(r,p,\pi)\leq \max_{\tilde p\in \cP} V(\brr(\tilde p,\pi),\tilde p,\pi) + \bar \epsilon\tag{Assumption~\ref{camara-asp:eps-robust}}\,.
    \end{align*}
    By combining these equations together, we have
    \begin{align*}
        &\EEs{y\sim \pi, I\sim \gamma(\cdot,y)}{V(r_I^{\bar \epsilon},p,y)} - \max_{\tilde p\in \cP} V(\brr(\tilde p,\pi),\tilde p,\pi) - \bar \epsilon \\
        \leq& M_1\left( \max_{(r_I)_{I\in \cI}}\EEs{y\sim \pi,I\sim \gamma(\cdot,y)}{U(r_I,p,y)}-\max_r U(r,p,\pi) \right)+\epsilon\,.
    \end{align*}
    Consider a distribution $\cD$ over $\pi$. In \cite{camara2020mechanisms}, the signal $I$ contains the forecast $\pi$, then we have
    \begin{align*}
         &\EEs{\pi\sim \cD}{\EEs{y\sim \pi, I\sim \gamma(\cdot,y)}{V(r_I^{\bar \epsilon},p,y)} - \max_{\tilde p\in \cP} V(\brr(\tilde p,\pi),\tilde p,\pi)} - \bar \epsilon \\
        \leq& M_1\EEs{\pi\sim \cD}{\left( \max_{(r_I)_{I\in \cI}}\EEs{y\sim \pi,I\sim \gamma(\cdot,y)}{U(r_I,p,y)}-\max_r U(r,p,\pi) \right)}+\epsilon\\
        =& M_1\max_{(r_I)_{I\in \cI}}\EEs{\pi\sim \cD}{\left( \EEs{y\sim \pi,I\sim \gamma(\cdot,y)}{U(r_I,p,y)}-\max_r U(r,p,\pi) \right)}+\epsilon
        \,.
    \end{align*}
\end{proof}

\begin{itemize}
    \item Assumption~\ref{asp:principal-cal} is weaker than full calibration.
    \item For both the proposed mechanism and the constant mechanism, when $\pip_t = \pip_\tau$, we have $(p_t,\rho_t)=(p_\tau,\rho_\tau)$.
    Assumption~\ref{asp-alt:no-internal-reg} assumes that
    \begin{equation*}
         \max_{h}\frac{1}{T}\sum_{t=1}^T (U(h(p_t,\rho_t,r_t),p_t, y_t) - U(r_t,p_t,y_t)) \leq \epsilon\,,
    \end{equation*}
    which is weaker than Assumption~\ref{camara-asp:fcir} as that $\pip_t = \pip_\tau$ implies that $(p_t,\rho_t) = (p_\tau,\rho_\tau)$.
    \item  Agent's utility margin (Assumption \ref{asp:utility-margin}) and alignment (Assumption~\ref{camara-asp:alignment}) are alternative assumptions to connect Principal's utility and Agent's utility.
    \item Assumption~\ref{asp:no-sec-info} looks to be stronger than Assumption~\ref{camara-asp:fer}. However, under full calibration,Assumption~\ref{asp:no-sec-info} is approximately equal to Assumption~\ref{camara-asp:fer}. Again, $\pip_t = \pip_\tau$ implies that $(p_t,\rho_t)=(p_\tau,\rho_\tau)$
    \begin{align*}
        &\max_{h}\frac{1}{T}\sum_{t=1}^T U(h(\pip_t),p_t, y_t)=\frac{1}{T}\sum_{\pi} \max_{r_\pi}\sum_{t:\pip_t = \pi} U(r_\pi,p_\pi, y_t)\\
        &=\frac{1}{T}\sum_{\pi} \max_{r_\pi}n_\pi U(r_\pi,p_\pi, \hat \pi_{\pi})\\
        &\approx_{(\text{full calibration})}\frac{1}{T}\sum_{\pi} \max_{r_\pi}\sum_{t:\pip_t = \pi} U(r_\pi,p_\pi, \pi)
        \\&= \frac{1}{T}\sum_{(p,r)\in \cP\times\cR}\sum_{\pi:p_\pi = p, \brr(p,\pi) =r}\max_{r_\pi}\sum_{t:\pip_t = \pi} U(r_\pi,p, \pi)\\
        &= \frac{1}{T}\sum_{(p,r)\in \cP\times\cR}n_{p,r} U(r,p, \pi_{p,r})\\
        &= \frac{1}{T}\sum_{(p,r)\in \cP\times\cR}\max_{\tilde r}n_{p,r} U(\tilde r,p, \pi_{p,r})\\
        &\approx_{(\text{full calibration})}\max_{h:\cP\times \cR\mapsto \cR} \frac{1}{T}\sum_{t=1}^T U(h(p_t, \rho_t),p_t,y_t)\,.
    \end{align*}   
    % \begin{align*}
    %     &\max_{h:\cP\times \cR\mapsto \cR} \frac{1}{T}\sum_{t=1}^T U(h(p_t, \rho_t),p_t,y_t) = \frac{1}{T}\sum_{(p,r)\in \cP\times \cR}n_{p,r} \max_{\tilde r_{p,r}}U(\tilde r_{p,r},p,\hat \pi_{p,r})\\
    %     \geq & \frac{1}{T}\sum_{(p,r)\in \cP\times \cR}n_{p,r} \max_{\tilde r_{p,r}}U(\tilde r_{p,r},p,\pi_{p,r}) - \abs{\cP}\abs{\cR}\alpha \tag{calibration error (Assumption~\ref{asp:principal-cal})}\\
    %     =& \frac{1}{T}\sum_{(p,r)\in \cP\times \cR}\sum_{\pi: \brp(\pi) = p, \brr(p,\pi) =r}\sum_{t:\pip_t = \pi} U(r,p,\pip_t) - \abs{\cP}\abs{\cR}\alpha\tag{linearity}\\
    %     =& \frac{1}{T}\sum_{(p,r)\in \cP\times \cR}\sum_{\pi: \brp(\pi) = p, \brr(p,\pi) =r}\max_{\tilde r}\sum_{t:\pip_t = \pi} U(\tilde r,p,\pip_t) - \abs{\cP}\abs{\cR}\alpha\tag{BR}\\
    %     =&\max_{h}\frac{1}{T}\sum_{t=1}^T U(h(\pip_t),p_t, y_t)
    % \end{align*}
\end{itemize}
\subsection{Unreasonableness of Assumptions in Theorem 2 of \cite{camara2020mechanisms}}
In Theorem~2 of \cite{camara2020mechanisms}, the $\pi_t$ is replaced with $p_t$ in the context. Again, they assumed bounded CIR, lower bounded ER and alignment.
\begin{assumption}[bounded CIR]
\begin{equation*}
    \max_{h}\frac{1}{T}\sum_{t=1}^T (U(h(p_t,r_t^*,(r_t^p)_{p\in\cP}),p_t, y_t) - U(r_t,p_t,y_t)) \leq \epsilon\,.
\end{equation*}    
\end{assumption}
\begin{assumption}[lower-bounded ER]
    \begin{equation*}
    \max_{h}\frac{1}{T}\sum_{t=1}^T (U(h(p_t),p_t, y_t) - U(r_t,p_t,y_t)) \geq -\tilde \epsilon\,.
\end{equation*} 
\end{assumption}
\paragraph{Lower-bounded ER can be too stringent.}
Consider an example of contract design, where the contract space $\cP =\{1.5,1.6\}$, the action space of the Agent is $\{\text{work}, \text{shirk}\}$, and the nature state space is $\{\text{medium}, \text{hard}\}$. When the job is medium, working leads to success while shirking leads to failure; when the job is hard, both working and shirking lead to failure. The value of a job is $2$ and the cost of working is $1$.

Suppose that $y_t = \text{medium}$ for $t=1,\ldots,\frac{T}{2}$, and $y_t = \text{hard}$ for $t=\frac{T}{2}+1,\ldots,T$.
The Principal's forecast is $\abs{\sum_{t=1}^{\frac{T}{2}}\pi_t - y_t}$ is small, i.e., $\pi_t\approx y_t$ for most $t\leq \frac{T}{2}$. This should be true for any ``good'' forecaster (which has to maintain small calibration error for $y_t =\text{medium}$ for all $t=1\ldots,T$). 
Thus, the Principal's forecast is $\abs{\sum_{t=\frac{T}{2}+1}^{T}\pi_t - y_t}$ is small, i.e., $\pi_t\approx y_t$ for most $t> \frac{T}{2}$.
Consider the extreme case where $\pi_t = y_t$ for all $t\in [T]$.
The best in hindsight action is shirking and the utility of Agent is $0$.
Lower bounded ER requires the Agent to gain close to $0$ utility only, which not only assumes that the Agent has no extra information but also further restricts the Agent's behavior.

%\section{Auxiliary Lemmas}
%\begin{lemma}
%An Agent is best-responding to some predictor $\epsilon$-calibrated on the feature set $F$ iff they have $\epsilon$ regret, where the context is the Agent's own actions and $F$. 
%\end{lemma}
%\begin{proof}
%We will first show that calibration implies no internal regret.
%The Agent's payoff under the state sequence $y$ and the policy sequence $p$ can be written as



%$$\sum_{i=1}^{T}U(r_{t},p_{t},y_{t}) = \sum_{t =1}^{T}\sum_{f \in \mathcal{F}}U(r_{t},p_{t},y_{t})\ind{}$$

%Where $n_{f}$ is the number of rounds from $t=1$ to $T$ in which the context is $f$. 

%If $r_{t}$ is determined by the Agent best-responding to some predictor which is $\epsilon$-calibrated on $f \in F$, then 
%$$\sum_{f \in \mathcal{F}}U(r_{t},p_{t},y_{t})n_{f} - \sum_{f \in \mathcal{F}}U(r^{*},p_{t},\pi_{f})n_{f}$$

  %  \begin{equation*}
  %  \frac{1}{T} \norm{\sum_{t=1}^T \ind{(p_t ,\rho_t, \brr(p,\pir_t)) = (p,r,\bar r)} (\pir_t -y_t)}_1 \leq \alpha.
%\end{equation*}

%\end{proof}


==> src/general-bkup.tex <==
\section{Best response to forecasts}
We consider the case where both the Principal and the agent have (possibly different) forecasts and they always treat their forecasts as the true underlying prior and best respond to them.
More specifically, the interaction protocol is described as follows.
\begin{protocol}[H]
    \caption{Principal-Agent Interaction at round $t$}
    \label{prot:interaction}
        \begin{algorithmic}[1]
            \State{The Principal has a forecast $\pip_t$ and best responds to $\pip_t$ by choosing policy $p_t = \brp(\pip_t)$.}
            \State{The Principal has a recommendation of action to the agent based on her forecast $\pip_t$, i.e., $\rho_t = \brr(p_t,\pip_t)$.} 
            \State{The Principal reveals $(p_t, \rho_t)$ to the agent.}
            \State{The agent takes action $r_t$.}
            \State{The nature state $y_t$ is revealed.}
        \end{algorithmic}
    \end{protocol}

\subsection{Agent follows Principal's recommendation -- best responds to Principal's forecast}
We start with the simplest case where the agent follows the Principal's recommendation.
\begin{assumption}[calibration of Principal's forecast.]\label{asp:principal-cal}
For any sequence of nature states $y_{1:T}$, assume that for both the proposed mechanism $\sigma^*$ and the fixed constant mechanisms $\{\sigma^p\}_{p\in \cP}$, the principle's forecast $\pip_{1:T}$ is calibrated on the selected policy $p_t^*$ and the action taken by the agent $r_t^*$. More specifically, let $E = \{S_{p,r}|(p,r)\in \cP\times \cR\} \cup \{S'_{p,r}|(p,r)\in \cP\times \cR\}$ where
\begin{equation*}
    S_{p,r} : = \{\pi| \brp(\pi) = p , \brr(p,\pi) =r\}\,,
\end{equation*}
and 
\begin{equation*}
    S'_{p,r} : = \{\pi|\brr(p,\pi) =r\}\,.
\end{equation*}
More specifically, there exists a small $\alpha>0$ such that for any $S\in E$,
\begin{equation*}
    \frac{1}{T} \norm{\sum_{t=1}^T \ind{\pip_t \in S} (\pip_t -y_t)}_1 \leq \alpha.
\end{equation*}
\end{assumption}

\begin{lemma}\label{lmm:regret-follow-recommendation}
Under Assumption~\ref{asp:principal-cal}, the Principal's regret is bounded when the agent follows the Principal's recommendation. More specifically, we have
    \begin{align*}
        \max_{p\in \cP} \frac{1}{T}\sum_{t=1}^T \left(V(\rho_t^p, p, y_t)-V(\rho_t^*, p^*_t, y_t)\right) \leq  2\abs{\cP}\abs{\cR}\alpha\,,
    \end{align*}
    where $\rho_t^p = \brr(p,\pip_t)$ and $\rho_t^* = \brr(p^*_t,\pip_t)$ are recommendations under constant mechanism $\sigma^p$ and the proposed mechanism $\sigma^*$ respectively.
\end{lemma}
\begin{proof}
For any $S\in E$, let $\calerr(\pip,S) = \frac{1}{T} \norm{\sum_{t:\pip_t\in S} (\pip_t-y_t)}_1$ denote the calibration error on $S$.
Let $\calerr(\pip) = \max\left(\sum_{p,r} \calerr(\pip,S_{p,r}), \max_{p}\sum_{r}\calerr(\pip,S'_{p,r})\right)$, which is upper bounded by $\abs{\cP}\abs{\cR}\alpha$ under Assumption~\ref{asp:principal-cal}.
For proposed mechanism $\sigma^*$, let $t\in (p,r)$ denote $t:(p_t^*,\rho_t^*) = (p,r)$. Let $n_{p,r} = \sum_{t=1}^T\ind{t\in (p,r)}$ denote the number of rounds in which $(p_t^*,\rho_t^*) = (p,r)$. 
Let $\hat \pi_{p,r} = \frac{1}{n_{p,r}}\sum_{t\in (p,r)} y_t$ denote the empirical distribution of states in these rounds and $\pip_{p,r} = \frac{1}{n_{p,r}}\sum_{t\in (p,r)} \pip_t$ denote the empirical distribution of the forecasts.
For constant mechanism $\sigma^p$, let $t\in (r)$ denote $t: \rho_t^p = r$. 
Then we have
    \begin{align*}
        &\sum_{t=1}^T V(\rho_t^*,p_t^*,y_t) \\
        =& \sum_{(p,r)\in \cP\times \cR} \sum_{t\in (p,r)} V(r,p,y_t)\\
        =& \sum_{(p,r)\in \cP\times \cR} n_{p,r} \inner{V(r,p,\cdot)}{\hat \pi_{p,r}} \\
        \geq & \sum_{(p,r)\in \cP\times \cR} \left(n_{p,r} \inner{V(r,p,\cdot)}{\pip_{p,r}} -T\cdot\calerr(\pip,S_{p,r})\right)\tag{{calibration on }$S_{p,r}$}\\
        = & \sum_{(p,r)\in \cP\times \cR} \sum_{t\in(p,r)} \inner{V(\brr(p,\pip_t),p,\cdot)}{\pip_t} -T\cdot\calerr(\pip)\\
        \geq& \sum_{(p,r)\in \cP\times \cR} \sum_{t\in(p,r)} \max_{p'\in\cP}\inner{V(\brr(p',\pip_t),p',\cdot)}{\pip_t} -T\cdot\calerr(\pip) \tag{{best response}}\\
        \geq& \max_{p'\in\cP} \sum_{t=1}^T \inner{V(\brr(p',\pip_t),p',\cdot)}{\pip_t} -T\cdot\calerr(\pip)\\
        =& \max_{p'\in\cP} \sum_{r}\sum_{t:\brr(p',\pip_t) =r} \inner{V(r,p',\cdot)}{\pip_t} -T\cdot\calerr(\pip)\\
        \geq & \max_{p'\in\cP} \sum_{r}\left(\sum_{t:\brr(p',\pip_t) =r} V(r,p',y_t) - T
        \cdot\calerr(\pip, S'_{p',r})\right) -T\cdot\calerr(\pip)\tag{calibration on $S'_{p',r}$}\\
        =& \max_{p'\in \cP}\sum_{t=1}^T V(\rho_t^{p'}, p',y_t)-2T\cdot\calerr(\pip)\,.
    \end{align*}
    Under Assumption~\ref{asp:principal-cal}, we have $2T\cdot\calerr(\pip) \leq 2\alpha T$. We are done with the proof.
\end{proof}

\subsection{Agent best respond to her own forecast}
The agent does not necessarily follow the Principal's recommendation.
Instead, the agent could have her own forecast of nature states and best responds to it.

\begin{assumption}[calibration of agent's forecast.]\label{asp:agent-cal}
Suppose that the agent has a forecast $\pir_{1:T}$. At round $t$, the agent best responds to $(p_t,\pir_t)$ by taking $r_t = \brr(p_t,\pir_t)$. For any sequence of nature states $y_{1:T}$ and any realized sequence of policies $p_{1:T}$,  
    the agent's forecast is calibrated on time steps $t$ where $p_t = p, \rho_t=\brr(p_t,\pip_t) = \rho$ and $\brr(p_t, \pir_t) =  r$ for all $(p,\rho, r) \in \cP\times \cR\times \cR$. More specifically, there exists a small $\alpha>0$ such that for all $(p,\rho, r)\in \cP\times \cR\times \cR$, 
    \begin{equation*}
    \frac{1}{T} \norm{\sum_{t=1}^T \ind{(p_t ,\rho_t, \brr(p,\pir_t)) = (p,\rho, r)} (\pir_t -y_t)}_1 \leq \alpha\,,
\end{equation*}
\end{assumption}

\begin{assumptionp}{\ref*{asp:agent-cal}$'$}[no internal regret for agent]\label{asp-alt:no-internal-reg}
Let $\eint$ be an upper bound on the internal regret with context of $(p_t,\rho_t, r_t)$ for the realized sequence of states $y_{1:T}$ and realized sequence of policies $p_{1:T}$ and recommendations $\rho_{1:T}$ generated by either the proposed mechanism or the constant mechanisms.
That is,
    \begin{equation*}        \ir(y_{1:T},p^*_{1:T},\rho^{*}_{1:T}):=\max_{h:\cP\times \cR\times \cR\mapsto \cR}\frac{1}{T}\sum_{t=1}^T (U(h(p^*_t,\rho^{*}_t,r^*_t),p^*_t, y_t) - U(r^*_t,p^*_t,y_t)) \leq \eint\,,
    \end{equation*}
    and for all $p\in \cP$,
    \begin{equation*}        \ir(y_{1:T},(p,\ldots,p),\rho^{p}_{1:T}):=\max_{h:\cP\times \cR\times \cR\mapsto \cR}\frac{1}{T}\sum_{t=1}^T (U(h(p,\rho^{p}_t,r^p_t),p, y_t) - U(r^p_t,p,y_t)) \leq \eint\,.
    \end{equation*}
    We assume that there exists a small $\eint$.
    % There exists a small $>0$ such that for any sequence of nature states $y_{1:T}$ and any realized sequence of policies $p_{1:T}$,  the agent's achieves no-internal regret, i.e.,
\end{assumptionp}
For the proposed mechanism $\sigma^*$, let 
    $$\ir^*_{p,\rho} = \max_{h:\cR\mapsto \cR}\sum_{t\in (p,\rho)} \left(U(h(r^*_t),p^*_t, y_t) - U(r^*_t,p^*_t,y_t)\right)$$
    denote the internal regret for the agent in the rounds where  $(p^*_t,\rho^{*}_t) = (p,\rho)$.
    For the fixed mechanism $\sigma^p$, let 
    $$\ir^p_{\rho} = \max_{h:\cR\mapsto \cR}\sum_{t\in (\rho)} \left(U(h(r^p_t),p, y_t) - U(r^p_t,p,y_t)\right)$$
    denote the internal regret for the agent in the rounds where $\rho^{p}_t =  \rho$.
% Let $\ir^*_{p,r} = \max_{h:\cR\mapsto \cR}\sum_{t\in (p,r)} U(h(r_t),p_t, y_t) - U(r_t,p_t,y_t)$ denote the internal regret for the agent for the time steps $(p_t,\rho_t) = (p,r)$.
% By Assumption~\ref{asp-alt:no-internal-reg}, we have $\sum_{p,r}\ir_{p,r} \leq \epsilon T$.
\begin{remark}
    Note that Assumption~\ref{asp-alt:no-internal-reg} is weaker than Assumption~\ref{asp:agent-cal}.
    When Assumption~\ref{asp:agent-cal} holds, we have the internal regret satisfying that
    \begin{align*}
        \ir(y_{1:T},p_{1:T},\rho_{1:T})=&\max_{h}\frac{1}{T}\sum_{t=1}^T (U(h(p_t,\rho_t,r_t),p_t, y_t) - U(r_t,p_t,y_t)) \\
        =& \frac{1}{T}\sum_{(p,\rho, r)\in \cP\times \cR\times \cR}n_{p,\rho, r}\max_{\tilde r_{p,\rho, r}}(U(\tilde r_{p,\rho, r},p, \hat \pi_{p,\rho, r}) - U(r,p,\hat \pi_{p,\rho, r}))\\
        \leq &\frac{1}{T}\sum_{(p,\rho, r)\in \cP\times \cR\times \cR}\sum_{t\in (p,\rho, r)}\max_{\tilde r_{p,\rho, r}}(U(\tilde r_{p,\rho, r},p, \pir_t) - U( r,p,\pir_t))+ 2\abs{\cP}\abs{\cR}^2\alpha\\
        =& 2\abs{\cP}\abs{\cR}^2\alpha\,.
    \end{align*}
    where $n_{p,\rho, r}=\abs{\{t|p_t = p, \rho_t = \rho, r_t = r\}} $ and $\hat \pi_{p,\rho, r} = \frac{1}{n_{p,\rho, r}}\sum_{t=1}^T y_t\ind{p_t = p, \rho_t = \rho, r_t = r}$.
\end{remark}
% the principal has a forecast $\pip_{1:T}$. At each round $t$, the principal best responds to $\pip_t$ by choosing policy 
% \begin{equation*}
%     p_t = \brp(\pip_t):= \argmax_{p\in\cP} V(\brr(p,\pip_t),p,\pip_t)\,.
% \end{equation*}
% The principal also has a guess on action taken by the agent, $\rho_t = \brr(p_t,\pip_t)$, which does not necessarily to be the true action taken by the agent.
% Suppose that $\pip_{1:T}$ is calibrated on 



% The agent does not necessarily follow $\rho_t$.
% Instead, the agent has her own forecast $\pir_{1:T}$ and she will best respond to $(p_t, \pir_t)$ by taking action $r_t = \brr(p_t, \pir_t)$. 


\begin{assumption}[agent has no secret information.]\label{asp:no-sec-info}
Let $\eneg$ be an upper bound on the negative cross-swap regret for the realized sequence of states $y_{1:T}$ and realized sequence of policies $p_{1:T}$ and recommendations $\rho_{1:T}$ generated by the proposed mechanism and constant mechanisms.
That is,
    \begin{equation*}
        \nr(y_{1:T},p^*_{1:T},\rho^{*}_{1:T}):=\frac{1}{T}\sum_{t=1}^T U(r^*_t,p^*_t,y_t)- \max_{h:\cP\times \cR\mapsto \cR} \frac{1}{T}\sum_{t=1}^T U(h(p^*_t, \rho^{*}_t),p^*_t,y_t) \leq\eneg\,,
    \end{equation*}
    and for all $p\in \cP$,
    \begin{equation*}
        \nr(y_{1:T},(p,\ldots,p),\rho^{p}_{1:T}):=\frac{1}{T}\sum_{t=1}^T U(r^p_t,p,y_t)- \max_{h:\cP\times \cR\mapsto \cR} \frac{1}{T}\sum_{t=1}^T U(h(p, \rho^{p}_t),p,y_t) \leq\eneg\,.
    \end{equation*}
    We assume that there exists a small $\eneg$.
\end{assumption}
For the proposed mechanism $\sigma^*$, let 
    $$\nr^*_{p,\rho} = \sum_{t\in (p,\rho) }U(r^*_t,p^*_t,y_t)-\max_{\tilde r}\sum_{t\in (p,\rho)}U(\tilde r,p_t,y_t)$$
    denote the negative regret for the agent for the time steps $(p^*_t,\rho^{*}_t) = (p,\rho)$.
For the constant mechanism $\sigma^p$, let
    $$\nr^{p}_{\rho} = \sum_{t\in (\rho) }U(r^p_t,p,y_t)-\max_{\tilde r}\sum_{t\in (\rho)}U(\tilde r,p,y_t)$$
    denote the negative regret for the agent for the time steps $\rho^{p}_t =  \rho$.
% Let the negative regret in $\{t|p_t = p, \rho_t =r\}$ be
% \begin{equation}
%     \nr_{p,r} := \sum_{t:p_t = p, \rho_t =r }U(r_t,p_t,y_t)-\max_{\tilde r}\sum_{t:p_t = p, \rho_t =r}U(\tilde r,p_t,y_t)\,.\label{eq:x-swap}
% \end{equation}
% Then we have $\sum_{p,r}\nr_{p,r} \leq \eneg T$ according to Assumption~\ref{asp:no-sec-info}.

A more intuitive and direct way to model ``no secret information'' is assuming that the agent cannot consistently outperforms the Principal's recommendation, i.e., 
    \begin{equation}
        \frac{1}{T}\sum_{t=1}^T U(r_t,p_t,y_t) - \frac{1}{T}\sum_{t=1}^T U(\rho_t,p_t,y_t) \leq\eneg\,.\label{eq:no-better-than-guess}
    \end{equation}
\begin{lemma}
    If the agent can't consistently outperforms the Principal's  recommendation (Eq~\eqref{eq:no-better-than-guess}), then Assumption~\ref{asp:no-sec-info} holds.
\end{lemma}

\begin{assumption}[agent's utility margin.]\label{asp:utility-margin}\todohs{relax the assumption to get rid the polynomial dependence on $\abs{\cP}\abs{\cR}$}
There exists a $\pmargin>0$ such that
for policy sequence $p_{1:T}$ and recommendation sequence $\rho_{1:T}$ generated by either the proposed mechanism or the constant mechanism , for all $(p,\rho, r)\in \cP\times \cR\times \cR$, 
either
\begin{equation*}
    n_{p,\rho, r}:=\abs{\{t|p_t = p, \rho_t = \rho, r_t = r\}} \leq \frac{1}{\pmargin^2}\,,
\end{equation*}
or
\begin{equation*}
    \abs{U(p,\bar r, \hat \pi_{p,\rho, r}) - U(p,r, \hat \pi_{p,\rho, r})}\geq \pmargin\,,
\end{equation*}
where $\hat \pi_{p,\rho, r} = \frac{1}{n_{p,\rho, r}}\sum_{t=1}^T y_t\ind{p_t = p, \rho_t = \rho, r_t = r}$.
\end{assumption}
\begin{remark}
    This assumption comes up from the distributional setting.
    In the distributional setting, there exists a prior distribution $\pi\in \Delta(\cY)$ such that $y_{1:T}\stackrel{\text{i.i.d.}}{\sim} \pi$.
    In this case, to distinguish $\rho\neq r$, we need to assume that for any $p,\rho \neq r$, $\abs{U(\rho,p,\pi) - U(r,p,\pi)} \geq 2\pmargin$.
    This would implies our Assumption~\ref{asp:utility-margin} since if $n_{p,\rho, r}>\frac{1}{\pmargin^2}$, we have $\abs{U(p,\bar r, \hat \pi_{p,\rho, r}) - U(p,r, \hat \pi_{p,\rho, r})}\geq \pmargin$ by concentration inequality.
\end{remark}
For $ r\neq \rho$, without Assumption~\ref{asp:utility-margin}, it is possible that the agent achieve the same utility by selecting either $r$ or $\rho$, which leads to different Principal's utilities.
To make an assumption on the connection between the Principal's utility and the agent utility, we can also make the following alternative assumption, which is a variant of Assumption~\ref{camara-asp:alignment}. 

Analogous to \cite{camara2020mechanisms}, we define a signal as well. Our signal is the triple of policy, recommendation and action, $I_t = (p_t,\rho_t,r_t)$.
Let $\cI$ denote the signal space.
% Let $\cI$ denote the signal space with $\abs{\cI} = \abs{\cR}$. For times steps $t$ and $\tau$, the signal $I_t=I_\tau$ implies that the agent would take the same action, i.e., $r_t = r_\tau$.
% All agent needs to do is selecting a mapping from the signal to the action.
For any prior distribution $\pi$, let $p^*(\pi)$ denote the policy deployed by the Principal when running the proposed mechanism $\sigma^*$.
In this work, $p^*(\pi) = \brp(\pi)$ is the best response. 




\begin{assumptionp}{\ref*{asp:utility-margin}$'$}[alignment]\label{asp-alt:alignment}
    For any $p\in \cP$ and any signal structure $\gamma(\cdot, y)\in \Delta(\cI)$, we say the respond $(r_I^\epsilon(p))_{I\in \cI}$ is $\epsilon$-approximately optimal iff 
    \begin{align*}
        \EEs{y\sim \pi}{\EEs{J\sim \gamma(\cdot, y)}{U(r_J^\epsilon(p), p,y)}} \geq \max_{(r_I)_{I\in \cI}}\EEs{y\sim \pi}{\EEs{J\sim \gamma(\cdot, y)}{U(r_J, p,y)}} -\epsilon\,.
    \end{align*}
    Let $\tilde r(p) \in \argmax_r \EEs{y\sim \pi}{U(r, p,y)}$ denote the optimal fixed respond without signal and $(\tilde r_I(p))_{I\in \cI} \in\argmax_{(r_I)_{I\in \cI}}\EEs{y\sim \pi}{\EEs{I\sim \gamma(\cdot, y)}{U(r_I, p,y)}}$ denote the optimal respond given the signal.
    We assume that there exists a constant $M_1>0$ such that for any $\epsilon$-approximately optimal responds $(r_I^\epsilon)_{I\in \cI}$,
    \begin{align}
        &V(\tilde r(p^*(\pi)), p^*(\pi), \pi)-\EEs{y\sim \pi}{\EEs{J\sim \gamma(\cdot, y)}{V(r_J^\epsilon(p^*(\pi)), p^*(\pi),y)}}\nonumber\\
        \leq& M_1 (\EEs{y\sim \pi}{\EEs{J\sim \gamma(\cdot, y)}{U(\tilde r_J(p^*(\pi)), p^*(\pi),y)}} - U(\tilde r(p^*(\pi)), p^*(\pi), \pi) ) + \epsilon\,.\label{eq:alignment}
    \end{align}
    and for any fixed policy $p\in \cP$,
    \begin{align*}
        \EEs{y\sim \pi}{\EEs{J\sim \gamma(\cdot, y)}{V(r_J^\epsilon(p), p,y)}}-V(\tilde r(p),\tilde p, \pi)\nonumber
        \leq M_1 (\EEs{y\sim \pi}{\EEs{J\sim \gamma(\cdot, y)}{U(\tilde r_J(p), p,y)}} -  U(\tilde r (p), p, \pi) ) +  \epsilon\,,
    \end{align*}
\end{assumptionp}
\begin{remark}
    To parse this assumption, we can decompose Eq~\eqref{eq:alignment} into two parts. 
    First, 
    \begin{align}
        &V(\tilde r(p^*(\pi)), p^*(\pi), \pi)-\EEs{y\sim \pi}{\EEs{J\sim \gamma(\cdot, y)}{V(\tilde r_J(p^*(\pi)), p^*(\pi),y)}}\nonumber\\
        \leq& M_1 (\EEs{y\sim \pi}{\EEs{J\sim \gamma(\cdot, y)}{U(\tilde r_J(p^*(\pi)), p^*(\pi),y)}} - U(\tilde r(p^*(\pi)), p^*(\pi), \pi) ))\,,\label{eq:alignment-exact-opt}
    \end{align}
    and 
    \begin{equation}
        \EEs{y\sim \pi}{\EEs{I\sim \gamma(\cdot, y)}{V(\tilde r_I(p^*(\pi)), p^*(\pi),y)}}-\EEs{y\sim \pi}{\EEs{I\sim \gamma(\cdot, y)}{V(r_I^\epsilon(p^*(\pi)), p^*(\pi),y)}}\leq \epsilon\,.\label{eq:align-approx}\,.
    \end{equation}
    Eq~\eqref{eq:alignment-exact-opt} together with Eq~\eqref{eq:align-approx} implies Eq~\eqref{eq:alignment}.
    % where $\bar r_I = \argmax_{r_I}\EEs{y\sim \pi}{\EEs{I\sim \gamma(\cdot, y)}{U(r_I, p^*(\pi),y)}}$. 
    
    Eq~\eqref{eq:alignment-exact-opt} assumes that if the agent's utility remains relatively unchanged when they optimize their action based on a given signal compared to the utility they would have obtained by selecting the best action in hindsight (i.e., without considering the signal), then the Principal's utility should also remain close. We only have one-sided inequality here as we only need this for the proof. 
    Consider an example of contract design example where the prior distribution $\pi$ is equally distributed over $\{\text{medium}, \text{hard}\}$. Shirking all the time achieves zero agent's utility  while working for medium tasks and working w.p. $(p-1)$ for hard tasks also achieves zero agent's utility.
    These two actions are indifferent to the agent.
    Eq~\eqref{eq:alignment-exact-opt} requires that the Principal's utility when the agent shirk all the time is not much worse than that when the agent work for medium tasks and $(p-1)$ for hard tasks.

    Eq~\eqref{eq:align-approx} assumes that $\epsilon$-approximation does not change the Principal's utility by much.
\end{remark}

% \begin{remark}
%     For some fixed $(p,r)$, let $\cD$ be a distribution over priors such that every $\pi\in \supp(\cD)$ satisfies that $\brr(p,\pi) = r$. Let $\supp(\gamma_\pi(y))\subset (p,r)\times \cR$.
%     Then the agent's utility gain given the information is
%     \begin{align*}
%         &\EEs{\pi\sim \cD}{\EEs{y\sim \pi}{\EEs{J\sim \gamma_\pi(\cdot, y)}{U(\tilde r_J(p,\cD), p,y)}} -  U(\tilde r(p,\cD), p, \pi)}\\
%         =& 
%     \end{align*}
% \end{remark}
% \begin{assumptionp}{\ref*{asp:utility-margin}$''$}\label{alt-asp:alignment-belief}
%     For any prior distribution $\pi$, the agent might have a different belief of the nature, i.e., a latent variable $z\sim \cD$ and then $y\sim \pi_z$. 
%     We assume that there exists a constant $M_1>0$ such that
%     \begin{align}
%         &V(\tilde r(p^*(\pi)), p^*(\pi), \pi)-\EEs{z\sim \cD}{\EEs{y\sim \pi_z}{V(r_z^\epsilon, p^*(\pi),y)}}\nonumber\\
%         \leq& M_1 (\EEs{z\sim \cD}{\EEs{y\sim \pi_z}{U( \brr(p^*(\pi),\pi_z), p^*(\pi),y)}} - U(\tilde r(p^*(\pi)), p^*(\pi), \pi) ) + \epsilon\,,
%     \end{align}
%     where $r_z^\epsilon$ is an $\epsilon$-approximate best respond to $(p^*(\pi),\pi_z)$.
%     For any fixed policy $p\in \cP$
%     \begin{align*}
%         &\EEs{z\sim \cD}{\EEs{y\sim \pi_z}{V(r_z^\epsilon(p), p,y)}}-\max_{\tilde p}V(\tilde r(\tilde p),\tilde p, \pi)\nonumber\\
%         \leq& M_1 (\EEs{z\sim \cD}{\EEs{y\sim \pi_z}{U(\brr(p,\pi_z), p,y)}} - U(\tilde r(p), p, \pi) ) +  \epsilon\,,
%     \end{align*}
%     where $r_z^\epsilon(p)$ is an $\epsilon$-approximate best respond to $(p,\pi_z)$.
% \end{assumptionp}
\begin{theorem}
    Under Assumptions~\ref{asp:principal-cal},\ref{asp:agent-cal},\ref{asp:no-sec-info}, and \ref{asp:utility-margin},  the Principal's regret satisfies that 
    \begin{equation*}
        \textrm{PR}(y_{1:T}) \leq \cO(\frac{\abs{\cP}\abs{\cR}^2 }{\pmargin^2}\alpha + \frac{\abs{\cP}\abs{\cR}^2 }{\pmargin^3T}+\frac{\epsilon}{\pmargin}).
    \end{equation*}
\end{theorem}
The proof of the theorem follows immediately by combining Lemma~\ref{lmm:regret-follow-recommendation} and the following lemma.
\begin{lemma}[the disagreement region is small.]\label{lmm:disagreement}
For any realized policies $p_{1:T}$ generated by the proposed mechanism $\sigma^*$ or the constant mechanism $\sigma^p$ and any sequence of nature states $y_{1:T}$, 
under Assumption~\ref{asp:no-sec-info} and \ref{asp:utility-margin} , we have
\begin{equation*}
     \sum_{t=1}^T \ind{\rho_t\neq r_t} = \cO\left(\frac{2\calerr(\pip) +2(1+\frac{1}{\pmargin})\calerr(\pir)+ \epsilon }{\pmargin}T+ \frac{\abs{\cP}\abs{\cR}^2}{\pmargin^3}\right)\,,
\end{equation*}
where 
$\calerr(\pir) = \frac{1}{T}\sum_{(p,\rho, r)}\norm{\sum_{t\in (p,\rho, r)} y_t - \pir_t}_1$ \\
and $\calerr(\pip) = \max\left(\sum_{p,r} \calerr(\pip,S_{p,r}), \max_{p}\sum_{r}\calerr(\pip,S'_{p,r})\right)$.
Here $t\in (p,\rho, r)$ represents that $t\in \{\tau\in [T]: p_\tau = p, \rho_\tau = r, r_\tau = \bar r\}$ and $t\in (p,r)$ represents that $t\in \{\tau\in [T]: p_\tau = p, \rho_\tau = r\}$.
\end{lemma}
\begin{proof}
% For any variable $x_{1:T}$, let $\sum_{t\in (p,r,\bar r)}x_t$ to denote $\sum_{t=1}^T \ind{(p_t,\rho_t,r_t)=(p,r,\bar r)} x_t$ and $\sum_{t\in (p,r)}x_t$ to denote $\sum_{t=1}^T \ind{(p_t,\rho_t)=(p,r)} x_t$.
Let $\hat \pi_{p,r,\bar r} = \frac{1}{n_{p,r,\bar r}} \sum_{t\in (p,r,\bar r)}y_t$ and $\pir_{p,r,\bar r} = \frac{1}{n_{p,r,\bar r}} \sum_{t\in (p,r,\bar r)}\pir_t$.
Let us define $\hat \pi_{p,r}, \pir_{p,r}$ and $\pip_{p,r}$ similarly.
Let $\calerr(\pir, p,r,\bar r) = \frac{1}{T}\norm{\sum_{t\in (p,r,\bar r)} (y_t - \pir_t)}_1 = \frac{n_{p,r,\bar r}}{T}\norm{ \hat \pi_{p,r,\bar r}-\pir_{p,r,\bar r} }_1$.

We can show that 
% \begin{align*}
%     \sum_{t=1}^T U(r_t,p_t,y_t) &= \sum_{(p,r,\bar r)\in \cP\times \cR\times \cR} \sum_{t\in (p,r,\bar r)} U(\bar r,p,y_t) \\
%     &= \sum_{(p,r,\bar r)\in \cP\times \cR\times \cR} n_{p,r,\bar r} \inner{U(\bar r,p,\cdot )}{\hat \pi_{p,r,\bar r}}\tag{linearity}\\
%     &\leq \sum_{(p,r,\bar r)\in \cP\times \cR\times \cR} n_{p,r,\bar r} \left (\inner{U(\bar r,p,\cdot )}{\pi_{p,r,\bar r}} + T\cdot\calerr(\pir, p,r,\bar r)\right)\tag{{calibration}}\\
%     &= \sum_{(p,r,\bar r)\in \cP\times \cR\times \cR} \sum_{t\in (p,r,\bar r)} \EEs{y\sim  \pir_t}{U(\bar r,p,y)} + T\cdot\calerr(\pir)T\\
%     &=\sum_{(p,r,\bar r)\in \cP\times \cR\times \cR} \max _{\tilde r\in \cR}\sum_{t\in (p,r,\bar r)} \EEs{y\sim  \pir_t}{U(\tilde r,p,y)} + T\cdot\calerr(\pir)T\,. \tag{{best respond}}
% \end{align*}
\begin{align}
    \sum_{t\in (p,r,\bar r)}U(\bar r,p,y_t)=&  n_{p,r,\bar r} \inner{U(\bar r,p,\cdot )}{\hat \pi_{p,r,\bar r}}\tag{linearity}\nonumber\\
    \geq&  n_{p,r,\bar r} \inner{U(\bar r,p,\cdot )}{\pi_{p,r,\bar r}} - T\cdot\calerr(\pir, p,r,\bar r)\tag{{calibration}}\nonumber\\
    % &=  \sum_{t\in (p,r,\bar r)} \EEs{y\sim  \pir_t}{U(\bar r,p,y)} + n_{p,r,\bar r}T\cdot\calerr(\pir, p,r,\bar r)\\
    =&\max _{\tilde r\in \cR}\sum_{t\in (p,r,\bar r)} \EEs{y\sim  \pir_t}{U(\tilde r,p,y)} -  T\cdot\calerr(\pir, p,r,\bar r) \tag{{best response}}\nonumber\\
    \geq& \sum_{t\in (p,r,\bar r)} \inner{U( r,p,\cdot)}{\pi_{p,r,\bar r}} - T\cdot\calerr(\pir, p,r,\bar r)\nonumber\\
    \geq& n_{p,r,\bar r}U( r,p,\hat \pi_{p,r,\bar r}) -  2T\cdot\calerr(\pir, p,r,\bar r)\,,\label{eq:no-swap}
\end{align}
where the last inequality applies calibration.
On the other hand, we have that 
\begin{align}
    \sum_{\bar r\in \cR}n_{p,r,\bar r}U( \bar r,p,\hat \pi_{p,r,\bar r})&=\sum_{t\in (p,r)} U(r_t,p_t,y_t)
    =\max_{\tilde r}\sum_{t\in (p,r)} U(\tilde r,p,y_t) + \nr_{p,r}\tag{Def of $\nr_{p,r}$ in Eq~\eqref{eq:x-swap}}\nonumber\\
    &=\max_{\tilde r}n_{p,r} U(\tilde r,p,\hat \pi_{p,r}) + \nr_{p,r}\nonumber\\
    &\leq \max_{\tilde r}n_{p,r} U(\tilde r,p,\pip_{p,r}) +T\cdot\calerr(\pip,p,r)+ \nr_{p,r}\tag{calibration}\nonumber\\
    &= \max_{\tilde r}\sum_{t\in (p,r)} U(\tilde r,p,\pip_t) +T\cdot\calerr(\pip,p,r)+ \nr_{p,r}\tag{linearity}\nonumber\\
    &= \sum_{t\in (p,r)} U(r,p,\pip_t) +T\cdot\calerr(\pip,p,r)+ \nr_{p,r}\tag{best response}\nonumber\\
    &\leq \sum_{t\in (p,r)}U(r,p,y_t) + 2T\cdot\calerr(\pip,p,r) + \nr_{p,r}\tag{calibration}\nonumber\\
     &= \sum_{\bar r\in \cR}n_{p,r,\bar r}U(r,p,\hat \pi_{p,r,\bar r}) + 2T\cdot\calerr(\pip,p,r) + \nr_{p,r}\label{eq:nonneg-xswap}
\end{align}
According to Assumption~\ref{asp:utility-margin}, for all $(p,r,\bar r)$, either $n_{p,r,\bar r}\leq \frac{1}{\pmargin^2}$ or $\abs{U(p,\bar r, \hat \pi_{p,r,\bar r}) - U(p,r, \hat \pi_{p,r,\bar r})}\geq \pmargin$.
There are three cases:
\begin{itemize}
    \item Case 0: $n_{p,r,\bar r}\leq \frac{1}{\pmargin^2}$.
    \item Case 1: $U(p,\bar r,\hat \pi_{p,r,\bar r}) - U(p,r,\hat \pi_{p,r,\bar r}) \leq -\pmargin$. According to Eq~\eqref{eq:no-swap}, we have
    \begin{equation*}
        n_{p,r,\bar r}\pmargin \leq 2T\cdot\calerr(\pir,p,r,\bar r)\,,
    \end{equation*}
    which implies that $ n_{p,r,\bar r} \leq \frac{2T\cdot\calerr(\pir,p,r,\bar r)}{\pmargin}$.
    \item Case 2: $U(p,\bar r,\hat \pi_{p,r,\bar r}) - U(p,r,\hat \pi_{p,r,\bar r}) \geq \pmargin$, then according to Eq~\eqref{eq:nonneg-xswap}, we have
    \begin{align*}
        &-\sum_{\bar r\in \cR}\ind{\text{case 2}}n_{p,r,\bar r}\pmargin + 2T\cdot\calerr(\pip,p,r) + \nr_{p,r}\\
        \geq& -\sum_{\bar r\in \cR}(\ind{\text{case 1}}+\ind{\text{case 0}})n_{p,r,\bar r}U( r,p,\hat \pi_{p,r,\bar r})\\
        \geq &-\sum_{\bar r\in \cR}\frac{2T\cdot\calerr(\pir,p,r,\bar r)}{\pmargin} - \frac{\abs{\cR}}{\pmargin^2}\,.
    \end{align*}
    Hence we have
    \begin{align*}
        \sum_{\bar r\in \cR}\ind{\text{case 2}}n_{p,r,\bar r} &\leq \frac{2T\cdot\calerr(\pip,p,r) + \nr_{p,r}+\sum_{\bar r\in \cR}\frac{2T\cdot\calerr(\pir,p,r,\bar r)}{\pmargin} +\frac{\abs{\cR}}{\pmargin^2}}{\pmargin}
    \end{align*}
\end{itemize}
By combining all three cases, we have
\begin{equation*}
    \sum_{p,r}\sum_{\bar r\neq r }n_{p,r,\bar r}\leq \frac{2\calerr(\pip) +2\calerr(\pir)+ \epsilon  + \frac{2\cdot\calerr(\pir)}{\pmargin} }{\pmargin}T+ \frac{\abs{\cP}\abs{\cR}^2}{\pmargin^3}+ \frac{2\cdot\calerr(\pir)}{\pmargin} T+\frac{\abs{\cP}\abs{\cR}^2}{\pmargin^2}\,.
\end{equation*}
\end{proof}
\begin{lemma}[the Principal's utility difference is small]\label{lmm:utility-difference}
    For any sequence of nature states $y_{1:T}$, under Assumption~\ref{asp:no-sec-info} and \ref{asp-alt:alignment} , we have
\begin{equation*}
     \frac{1}{T}\sum_{t=1}^T V(r_t^*,p_t^*,y_t)\geq \frac{1}{T}\sum_{t=1}^T V(\rho^{*}_t,p_t^*,y_t)-(M_1+1)T\eint-M_1T\eneg -(4M_1+2)\calerr(\pip)
\end{equation*}
and for all $p\in \cP$
\begin{equation*}
     \frac{1}{T}\sum_{t=1}^T V(r_t^p,p,y_t)\leq \frac{1}{T}\sum_{t=1}^T V(\rho^{p}_t,p,y_t)+2\calerr(\pip) +  (M_1+1)T\eint + M_1T \eneg
\end{equation*}
\end{lemma}
\begin{proof}
    
    
    
    \textbf{Proof of the first part.} 
    For each $(p,r)\in \cP\times \cR$, let the signal be the true action taken by the agent, i.e., $I_t = r_t^*$. Let the signal structure $\hat\gamma_{p,r}(\bar r, y) := \frac{\sum_{t\in (p,r)} \ind{I_t = \bar r, y_t = y}}{\sum_{t\in (p,r)} \ind{y_t = y}}$.
    \begin{align}
      \sum_{t=1}^TV(r^*_t,p^*_t,y_t) =& \sum_{(p,r)\in \cP\times \cR} \sum_{\bar r\in \cR} n_{p,r,\bar r}\sum_{t\in (p,r,\bar r)} V(\bar r, p, y_t)\nonumber\\
        = & \sum_{(p,r)\in \cP\times \cR}n_{p,r} \EEs{y\sim \hat \pi_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}\nonumber\\
        \geq & \sum_{(p,r)\in \cP\times \cR}n_{p,r} \EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}} - \calerr(\pip,p,r)\label{eq:int-step-cal}\,.
    \end{align}
    Now we want to apply Eq~\eqref{eq:alignment} to lower bound Eq~\eqref{eq:int-step-cal}. The reason to apply calibration in Eq~\eqref{eq:int-step-cal} is that $p = \brp(\pip_{p,r})$ and $p\neq \brp(\hat \pi_{p,r})$ and Eq~\eqref{eq:alignment} only works for $(p,\pi)$ satisfying that $p = \brp(\pi)$.
    \begin{align}
        &\EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{U(J,p,y)}} \geq \EEs{y\sim \hat \pi_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{U(J,p,y)}} -\norm{\pip_{p,r} - \hat \pi_{p,r}}_1\nonumber\\
        =& \max_{r_I} \EEs{y\sim \hat \pi_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{U(r_J,p,y)}}- \frac{1}{n_{p,r}}\ir^*_{p,r} -\norm{\pip_{p,r}  - \hat \pi_{p,r}}_1\nonumber\\
        \geq & \max_{r_I} \EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{U(r_J,p,y)}}- \frac{1}{n_{p,r}}\ir^*_{p,r} -2\norm{\pip_{p,r}  - \hat \pi_{p,r}}_1 \,. \label{eq:step1}
    \end{align}
    On the other hand, we have
    \begin{align}
    &\EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{U(J,p,y)}} - \max_{\tilde r}\EEs{y\sim \pip_{p,r}}{U(\tilde r,p,y)} \nonumber\\
    \leq& \EEs{y\sim \hat \pi_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{U(J,p,y)}} - \max_{\tilde r}\EEs{y\sim \hat \pi_{p,r}}{U(\tilde r,p,y)}+ 2\norm{\pip_{p,r}  - \hat \pi_{p,r}}_1\nonumber\\
    =& \frac{1}{n_{p,r}}\nr_{p,r}+2\norm{\pip_{p,r}  - \hat \pi_{p,r}}_1\,.\label{eq:step2}
    \end{align}
Combine Eq~\eqref{eq:step1} and \eqref{eq:step2}, we have
\begin{align}
    &\max_{r_I} \EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{U(r_J,p,y)}}-\max_{\tilde r}\EEs{y\sim \pip_{p,r}}{U(\tilde r,p,y)}\nonumber\\
    \leq&  \frac{1}{n_{p,r}}\nr^*_{p,r}+\frac{1}{n_{p,r}}\ir^*_{p,r} +4\norm{\pip_{p,r}  -\hat \pi_{p,r}}_1\label{eq:setp-utility-gap}
\end{align}
According to Assumption~\ref{asp-alt:alignment}, we have
\begin{align*}
    &\EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}\\
    \geq& V(r,p,\pip_{p,r})-M_1(\frac{1}{n_{p,r}}\ir^*_{p,r}+\frac{1}{n_{p,r}}\nr^*_{p,r} +4\norm{\pip_{p,r}  -\hat \pi_{p,r}}_1) - \frac{1}{n_{p,r}}\ir^*_{p,r} -2\norm{\pip_{p,r}  - \hat \pi_{p,r}}_1\,.
\end{align*}
Hence, we have
\begin{align*}
&\sum_{t=1}^TV(r^*_t,p^*_t,y_t) \\
    \geq & \sum_{(p,r)\in \cP\times \cR} n_{p,r}V(r,p,\pip_{p,r})-(M_1+1)\ir^*_{p,r}-M_1\nr^*_{p,r} -(4M_1+2)\calerr(\pip,p,r)\\
    =& \sum_{t=1}^TV(\rho^{*}_t,p^*_t,y_t) -(M_1+1)T\eint-M_1T\eneg -(4M_1+2)\calerr(\pip)\,.
\end{align*}
\textbf{Proof of the second part under Assumption~\ref{asp-alt:alignment}.} 
Similarly, for any fixed mechanism $\sigma^p$, let the signal be the true action taken by the agent, i.e., $I_t = r_t^p$. Let the signal structure $\hat\gamma_{p,r}(\bar r, y) := \frac{\sum_{t\in (p,r)} \ind{I_t = \bar r, y_t = y}}{\sum_{t\in (p,r)} \ind{y_t = y}}$.
Similar to Eq~\eqref{eq:step1} and Eq~\eqref{eq:setp-utility-gap}, we also have
\begin{align*}
        &\EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{U(J,p,y)}} \\
        \geq & \max_{r_I} \EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{U(r_J,p,y)}}- \frac{1}{n_{p,r}}\ir^p_{p,r} -2\norm{\pip_{p,r}  - \hat \pi_{p,r}}_1 \,. 
    \end{align*}
    and
\begin{align*}
    &\max_{r_I} \EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{U(r_J,p,y)}}-\max_{\tilde r}\EEs{y\sim \pip_{p,r}}{U(\tilde r,p,y)}\\
    \leq&  \frac{1}{n_{p,r}}\nr^p_{p,r}+\frac{1}{n_{p,r}}\ir^p_{p,r} +4\norm{\pip_{p,r}  -\hat \pi_{p,r}}_1\,.
\end{align*}
Then combining with Assumption~\ref{asp-alt:alignment}, we have
\begin{align}
    &\EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}\nonumber\\
    \leq& \EEs{y\sim \pip_{p,r}}{V(\tilde r(p),p,y)} + M_1(\frac{1}{n_{p,r}}\nr^p_{p,r}+\frac{1}{n_{p,r}}\ir^p_{p,r} +4\norm{\pip_{p,r}  -\hat \pi_{p,r}}_1) \nonumber\\
    &+ \frac{1}{n_{p,r}}\ir^p_{p,r} +2\norm{\pip_{p,r}  - \hat \pi_{p,r}}_1    
    \,.\label{eq:step3}
\end{align}
For the first term, we have
\begin{align*}
    &\EEs{y\sim \pip_{p,r}}{V(\tilde r( p),p,y)}=\EEs{y\sim \pip_{p,r}}{V(\brr(\tilde p, \pip_{p,r}), p,y)} \tag{defn of $\tilde r$}\\
    =& \frac{1}{n_{p,r}}\sum_{t\in (p,r)} V(\brr( p, \pip_{p,r}), p,\pip_t)= \frac{1}{n_{p,r}}\sum_{t\in (p,r)} V(r, p,\pip_t)
\end{align*}
Therefore, we have
\begin{align*}
    &\sum_{t=1}^TV(r^p_t,p,y_t) =\sum_{r}\sum_{t\in (p,r)}V(r^p_t,p,y_t)\\
    =& \sum_{r}n_r \EEs{y\sim \hat \pi_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}\\
    \leq & \sum_{r}n_r \EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}+ \calerr(\pip,p,r)\\
    \leq & \sum_{r}n_r \left(\EEs{y\sim \pip_{p,r}}{V(\tilde r(p),p,y)} + \frac{1}{n_{p,r}}M_1\nr^p_{p,r}+\frac{1}{n_{p,r}}(M_1+1)\ir^p_{p,r} +(4M_1+2)\norm{\pip_{p,r}  -\hat \pi_{p,r}}_1\right)\\
    &+ \calerr(\pip,p,r)\tag{Eq~\eqref{eq:step3}}\\
    = & \sum_{r}n_r \left(\EEs{y\sim \pip_{p,r}}{V(r,p,y)} + \frac{1}{n_{p,r}}M_1\nr^p_{p,r}+\frac{1}{n_{p,r}}(M_1+1)\ir^p_{p,r} +(4M_1+2)\norm{\pip_{p,r}  -\hat \pi_{p,r}}_1\right)\\
    &+ \calerr(\pip,p,r)\\
    % = &\sum_{r}n_r \left(\max_{\tilde p}\EEs{y\sim \hat \pi_{p,r}}{V(\tilde r(\tilde p),\tilde p,y)}+ M_1(\ir^p_{p,r} + \nr^p_{p,r}) + \ir^p_{p,r}\right)\\
    \leq &\sum_{t=1}^T V(\rho^{\tilde p}_t, p,y_t)  +  (M_1+1)T\eint + M_1T \eneg+(4M+4)\calerr(\pip)\,.
\end{align*}
\textbf{Proof of the second part under Assumption~\ref{asp-alt-ver2:alignment}.} \todohs{not finished}
Let $\cD$ be the empirical distribution of $\pip_t$ for $t\in (p,r)$.
Let the signal structure $\hat\gamma_\pi((p,r,\bar r), y) := \frac{\sum_{t:\pip_t=\pi} \ind{I_t = \bar r, y_t = y}}{\sum_{t:\pip_t=\pi} \ind{y_t = y}}$ and $\hat\gamma_{p,r}((p,r,\bar r), y) := \frac{\sum_{t\in (p,r)} \ind{I_t = \bar r, y_t = y}}{\sum_{t\in (p,r)} \ind{y_t = y}}$.
Then we have
\begin{align*}
        &\EEs{\pi\sim \cD, y\sim \pi}{\EEs{J\sim \hat \gamma_{\pi}(\cdot,y)}{U(\bar r,p,y)}}= \frac{1}{n_{p,r}}\sum_{\bar r\in \cR} n_{p,r,\bar r} U(\bar r,p,\pip_{p,r,\bar r})\\
        \geq & \frac{1}{n_{p,r}}\sum_{\bar r\in \cR} n_{p,r,\bar r} U(\bar r,p,\hat \pi_{p,r,\bar r})-\norm{\pip_{p,r}  - \hat \pi_{p,r}}_1\\
        \geq & \frac{1}{n_{p,r}}\sum_{\bar r\in \cR} n_{p,r,\bar r} U(\bar r,p,\hat \pi_{p,r,\bar r})-\norm{\pip_{p,r}  - \hat \pi_{p,r}}_1\\
        \geq & \max_{r_I} \EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{U(r_J,p,y)}}- \frac{1}{n_{p,r}}\ir^p_{p,r} -2\norm{\pip_{p,r}  - \hat \pi_{p,r}}_1 \,. 
    \end{align*}
    and
\begin{align*}
    &\max_{r_I} \EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{U(r_J,p,y)}}-\max_{\tilde r}\EEs{y\sim \pip_{p,r}}{U(\tilde r,p,y)}\\
    \leq&  \frac{1}{n_{p,r}}\nr^p_{p,r}+\frac{1}{n_{p,r}}\ir^p_{p,r} +4\norm{\pip_{p,r}  -\hat \pi_{p,r}}_1\,.
\end{align*}
Then combining with Assumption~\ref{asp-alt:alignment}, we have
\begin{align}
    &\EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}\nonumber\\
    \leq& \EEs{y\sim \pip_{p,r}}{V(\tilde r(p),p,y)} + M_1(\frac{1}{n_{p,r}}\nr^p_{p,r}+\frac{1}{n_{p,r}}\ir^p_{p,r} +4\norm{\pip_{p,r}  -\hat \pi_{p,r}}_1) \nonumber\\
    &+ \frac{1}{n_{p,r}}\ir^p_{p,r} +2\norm{\pip_{p,r}  - \hat \pi_{p,r}}_1    
    \,.\label{eq:step3}
\end{align}
For the first term, we have
\begin{align*}
    &\EEs{y\sim \pip_{p,r}}{V(\tilde r( p),p,y)}=\EEs{y\sim \pip_{p,r}}{V(\brr(\tilde p, \pip_{p,r}), p,y)} \tag{defn of $\tilde r$}\\
    =& \frac{1}{n_{p,r}}\sum_{t\in (p,r)} V(\brr( p, \pip_{p,r}), p,\pip_t)= \frac{1}{n_{p,r}}\sum_{t\in (p,r)} V(r, p,\pip_t)
\end{align*}
Therefore, we have
\begin{align*}
    &\sum_{t=1}^TV(r^p_t,p,y_t) =\sum_{r}\sum_{t\in (p,r)}V(r^p_t,p,y_t)\\
    =& \sum_{r}n_r \EEs{y\sim \hat \pi_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}\\
    \leq & \sum_{r}n_r \EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}+ \calerr(\pip,p,r)\\
    \leq & \sum_{r}n_r \left(\EEs{y\sim \pip_{p,r}}{V(\tilde r(p),p,y)} + \frac{1}{n_{p,r}}M_1\nr^p_{p,r}+\frac{1}{n_{p,r}}(M_1+1)\ir^p_{p,r} +(4M_1+2)\norm{\pip_{p,r}  -\hat \pi_{p,r}}_1\right)\\
    &+ \calerr(\pip,p,r)\tag{Eq~\eqref{eq:step3}}\\
    = & \sum_{r}n_r \left(\EEs{y\sim \pip_{p,r}}{V(r,p,y)} + \frac{1}{n_{p,r}}M_1\nr^p_{p,r}+\frac{1}{n_{p,r}}(M_1+1)\ir^p_{p,r} +(4M_1+2)\norm{\pip_{p,r}  -\hat \pi_{p,r}}_1\right)\\
    &+ \calerr(\pip,p,r)\\
    % = &\sum_{r}n_r \left(\max_{\tilde p}\EEs{y\sim \hat \pi_{p,r}}{V(\tilde r(\tilde p),\tilde p,y)}+ M_1(\ir^p_{p,r} + \nr^p_{p,r}) + \ir^p_{p,r}\right)\\
    \leq &\sum_{t=1}^T V(\rho^{\tilde p}_t, p,y_t)  +  (M_1+1)T\eint + M_1T \eneg+(4M+4)\calerr(\pip)\,.
\end{align*}
\end{proof}





\paragraph{Discussion on assumptions} Assumptions~\ref{asp:agent-cal} and \ref{asp:no-sec-info} are designed to restrict the behavior of the agent. Here we briefly discuss why these two assumptions are necessary in the following example. Consider an example of contract design where the contract space $\cP =\{1.5,1.6\}$, the action space of the agent/worker is $\{\text{work}, \text{shirk}\}$, and the nature state space is $\{\text{medium}, \text{hard}\}$. When the job is medium, working leads to success while shirking leads to failure; when the job is hard, both working and shirking lead to failure. The value of a job is $2$ and the cost of working is $1$. Suppose that the nature state $y_t = \text{medium}$ for odd $t$ and $y_t = \text{hard}$ for even $t$.
There are two candidate forecasts: 1) perfect forecast with $\pi_t = y_t$ for all $t$ and 2) mediocre forecast with $\pi_t = (0.5,0.5)$ for all $t$.
\begin{itemize}
    \item Is it enough to have agent's forecast be calibrated on $(p_t,\rho_t,r_t)$ instead of $(p_t,r_t)$? We can show a negative result if the agent is only calibrated on $(p_t,r_t)$.  Suppose that the Principal has a perfect forecast $\pip_t = y_t$ and then $p_t = 1.5$ for all $t$. 
    When the agent only has a mediocre forecast $\pir_t = (0.5,0.5)$ and then the agent will respond by $r_t = \text{shirk}$; when the agent also has the perfect forecast $\pir_t = y_t$, the agent will respond by $\text{work}$ iff. $y_t = \text{medium}$. 
    Both forecasts are calibrated on $(p_t,r_t)$.
    The Principal's regret will not vanish if the agent adopts the mediocre forecast for the proposed mechanism while adopts the perfect forecast for the constant mechanism of $1.6$.

    \item Why does the agent have to satisfy lower bounded cross-swap regret?
    Suppose that the Principal's forecast is the mediocre one while the agent's forecast can be mediocre or perfect. The agent can adopt the mediocre forecast for the proposed mechanism while adopts the perfect forecast for the constant mechanism.
\end{itemize}
\subsection{A set of alternative assumptions}
In this section, we propose a set of alternative assumptions to match the assumptions in \cite{camara2020mechanisms}.
The main difference in this subsection from the previous one is that the context is $(p_t,\rho_t,p^*_t,\rho^*_t, r_t)$ instead of $(p_t,\rho_t, r_t)$.  


\begin{assumptionp}{\ref*{asp:principal-cal}$'$}[finer calibration of Principal's forecast]\label{asp-alt:Principal-cal}
For any sequence of nature states $y_{1:T}$, assume that for both the proposed mechanism $\sigma^*$ and the fixed constant mechanisms $\{\sigma^p\}_{p\in \cP}$, the principle's forecast $\pip_{1:T}$ is calibrated conditional on $\pip_t\in S$ for all $S\in E'$, where $E = \{S_{p,r}|(p,r)\in \cP\times \cR\} \cup \{S''_{p,r,p',r'}|(p,r,p',r')\in \cP\times \cR\times \cP\times \cR\}$ where
\begin{equation*}
    S_{p,r} : = \{\pi| \brp(\pi) = p , \brr(p,\pi) =r\}\,,
\end{equation*}
and 
\begin{equation*}
    S''_{p,r,p',r'} : = \{\pi|\brp(\pi) = p' , \brr(p',\pi) =r',\brr(p,\pi) =r\}\,.
\end{equation*}
More specifically, there exists a small $\alpha>0$ such that for any $S\in E$,
\begin{equation*}
    \frac{1}{T} \norm{\sum_{t=1}^T \ind{\pip_t \in S} (\pip_t -y_t)}_1 \leq \alpha.
\end{equation*}
\end{assumptionp}

\begin{assumptionp}{\ref*{asp:agent-cal}$''$}[no finer counterfactual internal regret for agent]\label{asp-alt:no-finer-internal-reg}
Let $\eint$ be an upper bound on the internal regret with context of $(p_t,\rho_t, p^*_t, \rho^*_t, r_t)$ for the realized sequence of states $y_{1:T}$ and realized sequence of policies $p_{1:T}$ and recommendations $\rho_{1:T}$ generated by either the proposed mechanism or the constant mechanisms.
\end{assumptionp}

% \begin{assumption}[agent has no secret information.]\label{asp:no-sec-info}
% Let $\eneg$ be an upper bound on the negative cross-swap regret for the realized sequence of states $y_{1:T}$ and realized sequence of policies $p_{1:T}$ and recommendations $\rho_{1:T}$ generated by the proposed mechanism and constant mechanisms.
% That is,
%     \begin{equation*}
%         \nr(y_{1:T},p^*_{1:T},\rho^{*}_{1:T}):=\frac{1}{T}\sum_{t=1}^T U(r^*_t,p^*_t,y_t)- \max_{h:\cP\times \cR\mapsto \cR} \frac{1}{T}\sum_{t=1}^T U(h(p^*_t, \rho^{*}_t),p^*_t,y_t) \leq\eneg\,,
%     \end{equation*}
%     and for all $p\in \cP$,
%     \begin{equation*}
%         \nr(y_{1:T},(p,\ldots,p),\rho^{p}_{1:T}):=\frac{1}{T}\sum_{t=1}^T U(r^p_t,p,y_t)- \max_{h:\cP\times \cR\mapsto \cR} \frac{1}{T}\sum_{t=1}^T U(h(p, \rho^{p}_t),p,y_t) \leq\eneg\,.
%     \end{equation*}
%     We assume that there exists a small $\eneg$.
% \end{assumption}

\begin{assumptionp}{\ref*{asp:utility-margin}$''$}[alignment]\label{asp-alt-ver2:alignment}\todohs{not finished}
    We assume that there exists a constant $M_1>0$ such that for any $\epsilon$-approximately optimal responds $(r_I^\epsilon)_{I\in \cI}$,
    \begin{align}
        &V(\tilde r(p^*(\pi)), p^*(\pi), \pi)-\EEs{y\sim \pi}{\EEs{J\sim \gamma(\cdot, y)}{V(r_J^\epsilon(p^*(\pi)), p^*(\pi),y)}}\nonumber\\
        \leq& M_1 (\EEs{y\sim \pi}{\EEs{J\sim \gamma(\cdot, y)}{U(\tilde r_J(p^*(\pi)), p^*(\pi),y)}} - U(\tilde r(p^*(\pi)), p^*(\pi), \pi) ) + \epsilon\,.\label{eq:alignment}
    \end{align}
    and for any fixed policy $p\in \cP$,
    \begin{align*}
        \EEs{y\sim \pi}{\EEs{J\sim \gamma(\cdot, y)}{V(r_J^\epsilon(p), p,y)}}-\max_{p'\in \cP}V(\tilde r(p'),p', \pi)\nonumber
        \leq M_1 (\EEs{y\sim \pi}{\EEs{J\sim \gamma(\cdot, y)}{U(\tilde r_J(p), p,y)}} -  U(\tilde r (p), p, \pi) ) +  \epsilon\,,
    \end{align*}
\end{assumptionp}
\begin{theorem}
    Under Assumptions~\ref{asp-alt:principal-cal}, \ref{asp-alt:no-finer-internal-reg},\ref{asp:no-sec-info},\ref{asp-alt-ver2:alignment}, the principal achieves no regret.
\end{theorem}
\begin{proof}
    To prove the theorem, we will prove that
\begin{equation*}
     \frac{1}{T}\sum_{t=1}^T V(r_t^*,p_t^*,y_t)\geq \frac{1}{T}\sum_{t=1}^T V(\rho^{*}_t,p_t^*,y_t)-(M_1+1)T\eint-M_1T\eneg -(4M_1+2)\calerr(\pip)\,,
\end{equation*}
and for all $p\in \cP$
\begin{equation*}
     \frac{1}{T}\sum_{t=1}^T V(r_t^p,p,y_t)\leq \frac{1}{T}\sum_{t=1}^T V(\rho^{*}_t,p_t^*,y_t) +  (M_1+1)T\eint + M_1T \eneg\,.
\end{equation*}
The first part has been proved in Lemma~\ref{lmm:utility-difference}. We only need to prove the second part.
For any constant mechanism $\sigma^p$, now we consider the subsequence in which $\brp(\pip_t) = p' , \brr(p',\pip_t) =\rho',\brr(p,\pip_t) =\rho$. 
Let $t\in (p,\rho,p',\rho')$ to present $t: \brp(\pip_t) = p' , \brr(p',\pip_t) =\rho',\brr(p,\pip_t) =\rho$.
In this subsequence, we let the signal structure be $\hat\gamma_{p,\rho,p',\rho'}((p,\rho,r), y) := \frac{\sum_{t\in (p,\rho,p',\rho')} \ind{r^p_t = r, y_t = y}}{\sum_{t\in (p,\rho,p',\rho')} \ind{y_t = y}}$.
Then we have
\begin{align*}
        &\EEs{y\sim \pip_{p,\rho,p',\rho'}}{\EEs{J\sim \hat \gamma_{p,\rho,p',\rho'}(\cdot,y)}{U(r_J,p,y)}} \\
        \geq & \max_{r_I} \EEs{y\sim \pip_{p,\rho,p',\rho'}}{\EEs{J\sim \hat \gamma_{p,\rho,p',\rho'}(\cdot,y)}{U(r_J,p,y)}}- \frac{1}{n_{p,\rho,p',\rho'}}\ir^p_{p,\rho,p',\rho'} -2\norm{\pip_{p,\rho,p',\rho'}  - \hat \pi_{p,\rho,p',\rho'}}_1 \,. 
    \end{align*}
    and
\begin{align*}
    &\max_{r_I} \EEs{y\sim \pip_{p,\rho,p',\rho'}}{\EEs{J\sim \hat \gamma_{p,\rho,p',\rho'}(\cdot,y)}{U(r_J,p,y)}}-\max_{\tilde r}\EEs{y\sim \pip_{p,\rho,p',\rho'}}{U(\tilde r,p,y)}\\
    \leq&  \frac{1}{n_{p,\rho,p',\rho'}}\nr^p_{p,\rho,p',\rho'}+\frac{1}{n_{p,\rho,p',\rho'}}\ir^p_{p,\rho,p',\rho'} +4\norm{\pip_{p,\rho,p',\rho'}  -\hat \pi_{p,\rho,p',\rho'}}_1\,.
\end{align*}
Then combining with Assumption~\ref{asp-alt-ver2:alignment}, we have
\begin{align}
    &\EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}\nonumber\\
    \leq& \EEs{y\sim \pip_{p,r}}{V(\tilde r(p),p,y)} + M_1(\frac{1}{n_{p,r}}\nr^p_{p,r}+\frac{1}{n_{p,r}}\ir^p_{p,r} +4\norm{\pip_{p,r}  -\hat \pi_{p,r}}_1) \nonumber\\
    &+ \frac{1}{n_{p,r}}\ir^p_{p,r} +2\norm{\pip_{p,r}  - \hat \pi_{p,r}}_1    
    \,.\label{eq:step3}
\end{align}
For the first term, we have
\begin{align*}
    &\EEs{y\sim \pip_{p,r}}{V(\tilde r( p),p,y)}=\EEs{y\sim \pip_{p,r}}{V(\brr(\tilde p, \pip_{p,r}), p,y)} \tag{defn of $\tilde r$}\\
    =& \frac{1}{n_{p,r}}\sum_{t\in (p,r)} V(\brr( p, \pip_{p,r}), p,\pip_t)= \frac{1}{n_{p,r}}\sum_{t\in (p,r)} V(r, p,\pip_t)
\end{align*}
Therefore, we have
\begin{align*}
    &\sum_{t=1}^TV(r^p_t,p,y_t) =\sum_{r}\sum_{t\in (p,r)}V(r^p_t,p,y_t)\\
    =& \sum_{r}n_r \EEs{y\sim \hat \pi_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}\\
    \leq & \sum_{r}n_r \EEs{y\sim \pip_{p,r}}{\EEs{J\sim \hat \gamma_{p,r}(\cdot,y)}{V(J,p,y)}}+ \calerr(\pip,p,r)\\
    \leq & \sum_{r}n_r \left(\EEs{y\sim \pip_{p,r}}{V(\tilde r(p),p,y)} + \frac{1}{n_{p,r}}M_1\nr^p_{p,r}+\frac{1}{n_{p,r}}(M_1+1)\ir^p_{p,r} +(4M_1+2)\norm{\pip_{p,r}  -\hat \pi_{p,r}}_1\right)\\
    &+ \calerr(\pip,p,r)\tag{Eq~\eqref{eq:step3}}\\
    = & \sum_{r}n_r \left(\EEs{y\sim \pip_{p,r}}{V(r,p,y)} + \frac{1}{n_{p,r}}M_1\nr^p_{p,r}+\frac{1}{n_{p,r}}(M_1+1)\ir^p_{p,r} +(4M_1+2)\norm{\pip_{p,r}  -\hat \pi_{p,r}}_1\right)\\
    &+ \calerr(\pip,p,r)\\
    % = &\sum_{r}n_r \left(\max_{\tilde p}\EEs{y\sim \hat \pi_{p,r}}{V(\tilde r(\tilde p),\tilde p,y)}+ M_1(\ir^p_{p,r} + \nr^p_{p,r}) + \ir^p_{p,r}\right)\\
    \leq &\sum_{t=1}^T V(\rho^{\tilde p}_t, p,y_t)  +  (M_1+1)T\eint + M_1T \eneg+(4M+4)\calerr(\pip)\,.
\end{align*}
\end{proof}

